Model Averaging and Double Machine Learning

This paper discusses pairing double/debiased machine learning (DDML) with stacking, a model averaging method for combining multiple candidate learners, to estimate structural parameters. In addition to conventional stacking, we consider two stacking variants available for DDML: short-stacking exploits the cross-fitting step of DDML to substantially reduce the computational burden and pooled stacking enforces common stacking weights over cross-fitting folds. Using calibrated simulation studies and two applications estimating gender gaps in citations and wages, we show that DDML with stacking is more robust to partially unknown functional forms than common alternative approaches based on single pre-selected learners. We provide Stata and R software implementing our proposals.

==> GWG/Average_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 10:07:23 2023
 OLS/logit & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  OLS/logit (simple) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 3 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  

==> GWG/Average_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 10:18:19 2023
 OLS/logit & 0.077 & 0.077 & 0.077 \\ 
  OLS/logit (simple) & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso (extended) & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge (extended) & 0.077 & 0.077 & 0.077 \\ 
  Random forest 1 & 0.077 & 0.077 & 0.077 \\ 
  Random forest 2 & 0.077 & 0.077 & 0.077 \\ 
  Random forest 3 & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 1 & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 2 & 0.077 & 0.077 & 0.077 \\ 
  Neural net 1 & 0.077 & 0.077 & 0.077 \\ 
  Neural net 2 & 0.077 & 0.077 & 0.077 \\ 
  

==> GWG/Average_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 10:07:23 2023
 OLS/logit & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  OLS/logit (simple) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-lasso (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  CV-ridge (extended) & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Random forest 3 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Gradient boosting 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 1 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  Neural net 2 & 0.077 & 0.077 & 0.077 &  & 0.077 & 0.077 & 0.077 \\ 
  

==> GWG/CLS_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.023 & 0.012 & 0.242 &  & 0.014 & 0.001 & 0.257 &  & 0.027 & 0.013 & 0.211 \\ 
  OLS/logit (simple) & 0.004 & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.103 & 0.136 & 0.109 &  & 0.15\phantom{0} & 0.23\phantom{0} & 0.136 &  & 0.03\phantom{0} & 0.076 & 0.047 \\ 
  CV-ridge & 0.189 & 0.04\phantom{0} & 0.064 &  & 0.205 & 0.064 & 0.063 &  & 0.225 & 0.024 & 0.108 \\ 
  CV-lasso (extended) & 0.041 & 0.157 & 0.016 &  & 0.\phantom{000} & 0.078 & 0.\phantom{000} &  & 0.035 & 0.266 & 0.002 \\ 
  CV-ridge (extended) & 0.011 & 0.04\phantom{0} & 0.011 &  & 0.\phantom{000} & 0.019 & 0.\phantom{000} &  & 0.003 & 0.024 & 0.022 \\ 
  Random forest 1 & 0.435 & 0.506 & 0.275 &  & 0.462 & 0.521 & 0.288 &  & 0.483 & 0.507 & 0.28\phantom{0} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.025 & 0.008 & 0.039 &  & 0.\phantom{000} & 0.\phantom{000} & 0.008 &  & 0.011 & 0.003 & 0.022 \\ 
  Gradient boosting 2 & 0.15\phantom{0} & 0.059 & 0.216 &  & 0.165 & 0.071 & 0.23\phantom{0} &  & 0.175 & 0.063 & 0.285 \\ 
  Neural net 1 & 0.013 & 0.022 & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.008 & 0.02\phantom{0} & 0.027 &  & 0.004 & 0.016 & 0.018 &  & 0.01\phantom{0} & 0.023 & 0.023 \\ 
  

==> GWG/CLS_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.023 & 0.012 & 0.242 &  & 0.027 & 0.013 & 0.211 \\ 
  OLS/logit (simple) & 0.004 & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.103 & 0.136 & 0.109 &  & 0.03\phantom{0} & 0.076 & 0.047 \\ 
  CV-ridge & 0.189 & 0.04\phantom{0} & 0.064 &  & 0.225 & 0.024 & 0.108 \\ 
  CV-lasso (extended) & 0.041 & 0.157 & 0.016 &  & 0.035 & 0.266 & 0.002 \\ 
  CV-ridge (extended) & 0.011 & 0.04\phantom{0} & 0.011 &  & 0.003 & 0.024 & 0.022 \\ 
  Random forest 1 & 0.435 & 0.506 & 0.275 &  & 0.483 & 0.507 & 0.28\phantom{0} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.025 & 0.008 & 0.039 &  & 0.011 & 0.003 & 0.022 \\ 
  Gradient boosting 2 & 0.15\phantom{0} & 0.059 & 0.216 &  & 0.175 & 0.063 & 0.285 \\ 
  Neural net 1 & 0.013 & 0.022 & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.008 & 0.02\phantom{0} & 0.027 &  & 0.01\phantom{0} & 0.023 & 0.023 \\ 
  

==> GWG/Interactive_mse.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 Interactive & OLS/logit & 0.161 & 0.369 & 0.347 \\ 
  Interactive & OLS/logit (simple) & 0.223 & 0.267 & 0.204 \\ 
  Interactive & CV-lasso & 0.16\phantom{0} & 0.236 & 0.178 \\ 
  Interactive & CV-ridge & 0.161 & 0.237 & 0.18\phantom{0} \\ 
  Interactive & CV-lasso (extended) & 0.161 & 0.238 & 0.18\phantom{0} \\ 
  Interactive & CV-ridge (extended) & 0.161 & 0.336 & 0.194 \\ 
  Interactive & Random forest 1 & 0.161 & 0.23\phantom{0} & 0.176 \\ 
  Interactive & Random forest 2 & 0.171 & 0.258 & 0.19\phantom{0} \\ 
  Interactive & Random forest 3 & 0.179 & 0.274 & 0.199 \\ 
  Interactive & Gradient boosting 1 & 0.16\phantom{0} & 0.239 & 0.183 \\ 
  Interactive & Gradient boosting 2 & 0.161 & 0.254 & 0.196 \\ 
  Interactive & Neural net 1 & 0.241 & 0.349 & 0.263 \\ 
  Interactive & Neural net 2 & 0.176 & 0.643 & 0.357 \\ 
  

==> GWG/OLS_weights.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit &  0.022 & -0.01\phantom{0} &  0.206 &  &  0.009 & -0.008 &  0.212 &  &  0.039 & -0.006 &  0.193 \\ 
  OLS/logit (simple) & -0.035 & -0.019 &  0.081 &  & -0.041 & -0.014 &  0.083 &  & -0.072 & -0.019 &  0.075 \\ 
  CV-lasso &  0.007 & -0.024 &  0.326 &  &  0.056 &  0.078 &  0.202 &  & -0.222 & -0.154 &  0.169 \\ 
  CV-ridge &  0.534 &  0.28\phantom{0} &  0.089 &  &  0.462 &  0.295 &  0.105 &  &  0.709 &  0.33\phantom{0} &  0.204 \\ 
  CV-lasso (extended) & -0.028 &  0.251 & -0.189 &  & -0.056 &  0.123 & -0.081 &  &  0.041 &  0.378 & -0.2\phantom{00} \\ 
  CV-ridge (extended) & -0.086 & -0.049 &  0.015 &  & -0.042 & -0.045 &  0.008 &  & -0.149 & -0.075 &  0.024 \\ 
  Random forest 1 &  0.673 &  0.538 &  0.407 &  &  0.693 &  0.539 &  0.411 &  &  0.762 &  0.57\phantom{0} &  0.425 \\ 
  Random forest 2 & -0.098 &  0.383 &  0.112 &  & -0.06\phantom{0} &  0.411 &  0.11\phantom{0} &  & -0.035 &  0.143 &  0.124 \\ 
  Random forest 3 & -0.023 & -0.287 & -0.234 &  & -0.069 & -0.314 & -0.236 &  & -0.163 & -0.13\phantom{0} & -0.267 \\ 
  Gradient boosting 1 &  0.039 & -0.051 &  0.088 &  &  0.039 & -0.042 &  0.087 &  &  0.058 &  0.005 &  0.089 \\ 
  Gradient boosting 2 &  0.084 &  0.045 &  0.154 &  &  0.085 &  0.046 &  0.156 &  &  0.088 &  0.028 &  0.216 \\ 
  Neural net 1 & -0.312 & -0.158 & -1.635 &  &  0.001 &  0.011 & -0.005 &  &  0.001 &  0.028 & -0.052 \\ 
  Neural net 2 & -0.005 &  0.007 &  0.021 &  & -0.004 &  0.011 &  0.019 &  & -0.003 &  0.009 &  0.01\phantom{0} \\ 
  

==> GWG/OLS_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit &  0.009 & -0.008 &  0.212 \\ 
  OLS/logit (simple) & -0.041 & -0.014 &  0.083 \\ 
  CV-lasso &  0.056 &  0.078 &  0.202 \\ 
  CV-ridge &  0.462 &  0.295 &  0.105 \\ 
  CV-lasso (extended) & -0.056 &  0.123 & -0.081 \\ 
  CV-ridge (extended) & -0.042 & -0.045 &  0.008 \\ 
  Random forest 1 &  0.693 &  0.539 &  0.411 \\ 
  Random forest 2 & -0.06\phantom{0} &  0.411 &  0.11\phantom{0} \\ 
  Random forest 3 & -0.069 & -0.314 & -0.236 \\ 
  Gradient boosting 1 &  0.039 & -0.042 &  0.087 \\ 
  Gradient boosting 2 &  0.085 &  0.046 &  0.156 \\ 
  Neural net 1 &  0.001 &  0.011 & -0.005 \\ 
  Neural net 2 & -0.004 &  0.011 &  0.019 \\ 
  

==> GWG/OLS_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit &  0.022 & -0.01\phantom{0} &  0.206 &  &  0.039 & -0.006 &  0.193 \\ 
  OLS/logit (simple) & -0.035 & -0.019 &  0.081 &  & -0.072 & -0.019 &  0.075 \\ 
  CV-lasso &  0.007 & -0.024 &  0.326 &  & -0.222 & -0.154 &  0.169 \\ 
  CV-ridge &  0.534 &  0.28\phantom{0} &  0.089 &  &  0.709 &  0.33\phantom{0} &  0.204 \\ 
  CV-lasso (extended) & -0.028 &  0.251 & -0.189 &  &  0.041 &  0.378 & -0.2\phantom{00} \\ 
  CV-ridge (extended) & -0.086 & -0.049 &  0.015 &  & -0.149 & -0.075 &  0.024 \\ 
  Random forest 1 &  0.673 &  0.538 &  0.407 &  &  0.762 &  0.57\phantom{0} &  0.425 \\ 
  Random forest 2 & -0.098 &  0.383 &  0.112 &  & -0.035 &  0.143 &  0.124 \\ 
  Random forest 3 & -0.023 & -0.287 & -0.234 &  & -0.163 & -0.13\phantom{0} & -0.267 \\ 
  Gradient boosting 1 &  0.039 & -0.051 &  0.088 &  &  0.058 &  0.005 &  0.089 \\ 
  Gradient boosting 2 &  0.084 &  0.045 &  0.154 &  &  0.088 &  0.028 &  0.216 \\ 
  Neural net 1 & -0.312 & -0.158 & -1.635 &  &  0.001 &  0.028 & -0.052 \\ 
  Neural net 2 & -0.005 &  0.007 &  0.021 &  & -0.003 &  0.009 &  0.01\phantom{0} \\ 
  

==> GWG/Single-best_weights_onlypooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  OLS/logit (simple) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.\phantom{000} & 0.\phantom{000} & 1.\phantom{000} \\ 
  CV-ridge & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-ridge (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 1 & 1.\phantom{000} & 1.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  

==> GWG/Single-best_weights_wopooled.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 11:33:51 2023
 OLS/logit & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  OLS/logit (simple) & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  CV-lasso & 0.06\phantom{0} & 0.03\phantom{0} & 0.79\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.4\phantom{00} \\ 
  CV-ridge & 0.07\phantom{0} & 0.\phantom{000} & 0.04\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.1\phantom{00} \\ 
  CV-lasso (extended) & 0.02\phantom{0} & 0.06\phantom{0} & 0.03\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.1\phantom{00} \\ 
  CV-ridge (extended) & 0.\phantom{000} & 0.\phantom{000} & 0.01\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 1 & 0.85\phantom{0} & 0.91\phantom{0} & 0.02\phantom{0} &  & 1.\phantom{000} & 1.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Random forest 3 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Gradient boosting 1 & 0.\phantom{000} & 0.\phantom{000} & 0.11\phantom{0} &  & 0.\phantom{000} & 0.\phantom{000} & 0.4\phantom{00} \\ 
  Gradient boosting 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 1 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  Neural net 2 & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} & 0.\phantom{000} \\ 
  

==> GWG/regression_results_1.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 19:32:00 2023
estimator & avg & nnls1 & ols & singlebest \\ 
 Regular
stacking & -0.101 & -0.075 & -0.197 & -0.061 \\ 
   & (0.017)* & (0.028)* & (11.894) & (0.069) \\ 
  Short-
stacking & -0.101 & -0.076 & -0.001 & -0.085 \\ 
   & (0.017)* & (0.028)* & (0.184) & (0.065) \\ 
  Pooled
stacking & -0.101 & -0.075 & 0.137 & -0.072 \\ 
   & (0.017)* & (0.027)* & (0.111) & (0.055) \\ 
  

==> GWG/regression_results_2.tex <==
% latex table generated in R 4.3.2 by xtable 1.8-4 package
% Mon Dec 11 19:32:00 2023
estimator & indiv \\ 
 OLS/logit & -0.12 \\ 
   & (0.094) \\ 
  CV-lasso & -0.067 \\ 
   & (0.063) \\ 
  CV-ridge & -0.064 \\ 
   & (0.09) \\ 
  OLS/logit
(simple) & -0.12 \\ 
   & (0.016)* \\ 
  CV-lasso
(extended) & -0.055 \\ 
   & (0.076) \\ 
  CV-ridge
(extended) & -0.173 \\ 
   & (0.19) \\ 
  Random
forest 1 & -0.079 \\ 
   & (0.023)* \\ 
  Random
forest 2 & -0.105 \\ 
   & (0.016)* \\ 
  Random
forest 3 & -0.11 \\ 
   & (0.015)* \\ 
  Gradient
boosting 1 & -0.075 \\ 
   & (0.021)* \\ 
  Gradient
boosting 2 & -0.044 \\ 
   & (0.044) \\ 
  Neural
net 1 & -0.121 \\ 
   & (0.077) \\ 
  Neural
net 2 & -0.004 \\ 
   & (0.344) \\ 
  

==> Simul/not_selected.tex <==
1000&32951&.1&.1&1.7&895&415&417&415&902&900 \tabularnewline
1000&164755&.1&.1&1.7&258&769&769&769&258&258 \tabularnewline
1000&329509&.1&.1&1.7&2&618&618&618&2&2 \tabularnewline


==> Simul/sim_Advantages/sim_output_dgp0_10folds_withse.tex <==
&OLS&230.4&272.9&-28.4&198.8&9.7&140.9&11.7&102.0&78.3&39.1 \tabularnewline
&PDS-Lasso&-714.3&270.5&-739.5&197.3&-367.9&141.1&-76.3&102.3&78.8&39.1 \tabularnewline
&OLS&179.4&275.7&-85.1&199.2&2.5&141.0&7.9&102.0&77.8&39.1 \tabularnewline
&Lasso with CV (2nd order poly)&357.0&271.3&-38.9&199.6&3.4&141.7&9.1&102.1&77.5&39.1 \tabularnewline
&Ridge with CV (2nd order poly)&334.6&267.0&6.4&197.5&10.8&142.0&-9.9&102.0&77.5&39.2 \tabularnewline
&Lasso with CV (10th order poly)&-4864.6&5369.1&754.7&957.7&-476.8&1663.2&-547.1&454.5&141.0&46.4 \tabularnewline
&Ridge with CV (10th order poly)&-14274.3&10353.7&1038.4&7241.9&1596.6&3409.3&1442.5&1128.7&449.8&62.2 \tabularnewline
&Random forest (low regularization)&328.1&302.1&-112.2&220.3&-148.4&153.2&-69.6&112.1&-41.8&45.7 \tabularnewline
&Random forest (high regularization)&1086.7&274.9&255.6&201.6&206.3&143.1&128.5&103.7&68.4&39.9 \tabularnewline
&Gradient boosting (low regularization)&171.1&300.8&-280.4&210.3&-149.1&145.7&-60.3&104.2&44.3&39.3 \tabularnewline
&Gradient boosting (high regularization)&389.4&286.4&-77.4&203.4&65.0&142.9&75.2&102.6&139.1&39.2 \tabularnewline
&Neural net&3887.7&247.4&3926.3&199.2&3504.2&143.1&1874.9&104.9&212.1&39.2 \tabularnewline
&Stacking: CLS&-1150.3&1159.2&-84.3&224.9&28.2&165.0&47.1&111.1&73.1&39.2 \tabularnewline
&Stacking: Average&-3471.2&3073.6&195.7&358.6&-71.7&357.8&368.6&204.4&86.3&39.3 \tabularnewline
&Stacking: OLS&4.2e6&5.4e6&-1040.5&2688.0&-2085.4&1149.5&-365.2&255.9&32.8&55.8 \tabularnewline
&Stacking: Single-best&-5.0&275.9&-212.2&211.7&-57.8&141.7&-27.6&102.4&68.2&39.1 \tabularnewline
&Short-stacking: CLS&322.3&271.8&-54.8&199.6&51.6&141.2&25.1&102.1&73.2&39.1 \tabularnewline
&Short-stacking: Average&-3471.2&3073.6&195.7&358.6&-71.7&357.8&368.6&204.4&86.3&39.3 \tabularnewline
&Short-stacking: OLS&-214.9&269.4&-278.5&200.0&-100.4&140.4&-41.0&101.6&70.7&39.1 \tabularnewline
&Short-stacking: Single-best&189.1&271.1&-91.4&199.1&0.7&140.8&3.1&101.9&75.9&39.1 \tabularnewline
&Pooled stacking: CLS&465.6&271.7&39.7&199.8&89.6&140.9&18.0&102.1&73.7&39.1 \tabularnewline
&Pooled stacking: Average&-3471.2&3073.6&195.7&358.6&-71.7&357.8&368.6&204.4&86.3&39.3 \tabularnewline
&Pooled stacking: OLS&326.6&272.8&-97.4&200.0&-68.3&141.3&-23.2&102.3&72.6&39.1 \tabularnewline
&Pooled stacking: Single-best&150.8&270.7&-93.1&199.3&-11.6&141.2&8.3&102.1&76.6&39.1 \tabularnewline


==> Simul/sim_Advantages/sim_output_dgp0_2folds_withse.tex <==
&OLS&-67.4&277.9&190.0&204.8&-24.4&139.6&155.3&96.5&49.9&39.6 \tabularnewline
&PDS-Lasso&-1126.6&279.4&-577.4&203.9&-431.5&139.2&66.8&96.5&48.4&39.6 \tabularnewline
&OLS&-53.0&320.7&236.6&221.8&-22.0&148.2&186.4&99.3&46.2&39.7 \tabularnewline
&Lasso with CV (2nd order poly)&345.5&294.7&262.7&212.0&5.7&145.0&193.5&98.4&50.9&39.7 \tabularnewline
&Ridge with CV (2nd order poly)&313.7&287.6&293.8&208.9&120.1&142.4&213.8&98.7&48.2&39.9 \tabularnewline
&Lasso with CV (10th order poly)&25276.6&25779.0&-1632.0&3244.5&742.4&1948.5&1470.1&864.2&248.1&266.6 \tabularnewline
&Ridge with CV (10th order poly)&7927.1&9354.4&-267.5&6531.6&6359.4&5589.5&2776.4&2141.1&1230.1&401.8 \tabularnewline
&Random forest (low regularization)&240.3&314.1&89.3&232.8&-255.9&156.1&22.4&113.1&-74.7&48.6 \tabularnewline
&Random forest (high regularization)&2159.2&288.2&999.1&212.2&332.8&144.3&355.0&100.5&69.1&41.7 \tabularnewline
&Gradient boosting (low regularization)&-167.8&319.3&-85.0&234.7&-294.2&151.7&89.2&102.1&12.1&40.1 \tabularnewline
&Gradient boosting (high regularization)&129.5&305.6&169.1&221.8&-64.4&145.9&252.6&99.6&114.8&39.8 \tabularnewline
&Neural net&4241.3&304.3&4422.9&242.2&4260.5&174.1&3536.2&122.9&394.2&43.1 \tabularnewline
&Stacking: CLS&6329.4&5587.9&-66.9&531.5&-21.5&200.4&261.0&111.9&42.8&40.2 \tabularnewline
&Stacking: Average&-972.6&2751.4&1796.8&1765.4&254.6&647.7&815.2&215.7&107.7&51.2 \tabularnewline
&Stacking: OLS&-10699.3&13002.6&3.8e7&3.8e7&-63.3&2752.6&-1043.6&547.8&-129.3&96.2 \tabularnewline
&Stacking: Single-best&5893.9&5319.3&73.8&249.9&-158.5&149.5&115.1&99.1&43.7&39.9 \tabularnewline
&Short-stacking: CLS&389.3&285.0&314.6&210.6&9.9&144.1&218.4&98.2&45.0&39.7 \tabularnewline
&Short-stacking: Average&-972.6&2751.4&1796.8&1765.4&254.6&647.7&815.2&215.7&107.7&51.2 \tabularnewline
&Short-stacking: OLS&-207.9&275.1&84.7&206.1&-113.2&141.6&124.9&97.9&37.6&39.6 \tabularnewline
&Short-stacking: Single-best&241.8&284.2&209.2&210.2&-37.5&145.1&178.8&98.5&44.4&39.7 \tabularnewline
&Pooled stacking: CLS&-22063.1&22632.2&378.9&322.2&-141.5&166.8&230.4&107.1&58.6&41.4 \tabularnewline
&Pooled stacking: Average&-972.6&2751.4&1796.8&1765.4&254.6&647.7&815.2&215.7&107.7&51.2 \tabularnewline
&Pooled stacking: OLS&-26101.3&29649.6&-2324.4&2415.4&-1641.0&1777.9&-79.0&272.3&46.5&47.8 \tabularnewline
&Pooled stacking: Single-best&12247.4&12403.7&122.1&214.6&-88.2&146.2&156.7&98.6&46.9&39.7 \tabularnewline


==> Simul/sim_Advantages/sim_output_dgp1_10folds_withse.tex <==
&OLS&-2339.8&331.6&-2208.9&226.7&-2332.7&165.1&-2440.2&112.5&-2586.2&47.6 \tabularnewline
&PDS-Lasso&-2281.9&329.6&-2740.9&224.9&-2789.1&168.4&-2716.2&114.1&-2597.3&47.7 \tabularnewline
&OLS&-2864.1&370.5&-2607.8&247.4&-2479.6&172.1&-2526.7&115.0&-2606.5&47.8 \tabularnewline
&Lasso with CV (2nd order poly)&-1048.1&357.5&-730.3&232.5&243.2&166.1&467.6&111.8&783.4&43.0 \tabularnewline
&Ridge with CV (2nd order poly)&-1730.2&348.3&-1127.8&232.0&481.5&170.6&833.2&113.3&806.7&43.0 \tabularnewline
&Lasso with CV (10th order poly)&22248.8&25988.5&-2907.1&2774.5&1598.1&3131.5&4485.9&3456.2&185.6&457.2 \tabularnewline
&Ridge with CV (10th order poly)&24105.0&16649.8&2351.6&2060.6&-5341.5&5329.5&-602.5&2313.4&2873.4&552.4 \tabularnewline
&Random forest (low regularization)&-84.4&343.4&18.2&231.6&-5.4&158.3&-89.8&113.2&-63.6&47.7 \tabularnewline
&Random forest (high regularization)&-159.0&333.3&-37.4&223.1&99.8&154.6&-77.1&107.6&-78.1&42.7 \tabularnewline
&Gradient boosting (low regularization)&-281.5&351.7&-32.4&238.7&-11.1&157.8&34.1&108.8&64.6&41.3 \tabularnewline
&Gradient boosting (high regularization)&-89.7&336.4&208.6&229.0&179.2&152.6&182.9&105.2&218.2&41.2 \tabularnewline
&Neural net&1839.2&299.8&2045.7&225.2&1735.2&159.0&209.6&107.6&-472.8&43.6 \tabularnewline
&Stacking: CLS&11936.9&14230.0&-1198.8&965.2&803.6&583.6&915.4&1141.7&437.8&46.8 \tabularnewline
&Stacking: Average&7161.2&5979.0&498.4&566.1&-368.8&751.2&765.1&482.6&451.8&50.7 \tabularnewline
&Stacking: OLS&-2.7e7&2.4e7&-3391.9&2466.9&3033.6&3386.2&6271.2&4906.4&608.4&190.2 \tabularnewline
&Stacking: Single-best&3472.5&4282.0&-385.1&306.5&687.0&541.4&542.5&255.2&154.1&46.1 \tabularnewline
&Short-stacking: CLS&-278.6&311.4&-117.9&208.7&88.3&146.0&188.6&101.9&157.7&41.0 \tabularnewline
&Short-stacking: Average&7161.2&5979.0&498.4&566.1&-368.8&751.2&765.1&482.6&451.8&50.7 \tabularnewline
&Short-stacking: OLS&-524.0&298.3&-209.4&199.9&16.5&142.2&88.7&100.2&126.1&40.8 \tabularnewline
&Short-stacking: Single-best&-602.8&310.3&-363.9&215.6&51.5&150.3&196.2&104.5&66.9&41.3 \tabularnewline
&Pooled stacking: CLS&-382.2&315.4&-319.7&218.0&-73.3&150.7&143.9&103.7&179.9&41.0 \tabularnewline
&Pooled stacking: Average&7161.2&5979.0&498.4&566.1&-368.8&751.2&765.1&482.6&451.8&50.7 \tabularnewline
&Pooled stacking: OLS&-217.6&359.4&-231.1&223.5&-223.3&158.8&-23.4&120.8&152.0&40.9 \tabularnewline
&Pooled stacking: Single-best&-679.0&319.8&-316.5&228.0&-52.0&154.5&159.4&105.9&68.2&41.2 \tabularnewline


==> Simul/sim_Advantages/sim_output_dgp1_2folds_withse.tex <==
&OLS&-1890.5&320.1&-2398.9&226.0&-2645.8&174.3&-2793.8&120.9&-2588.9&46.5 \tabularnewline
&PDS-Lasso&-2001.6&321.4&-2953.3&230.4&-3105.9&177.2&-3078.5&122.1&-2598.7&46.5 \tabularnewline
&OLS&-2466.6&410.7&-2861.0&267.6&-2993.2&194.8&-2886.0&129.9&-2613.0&47.5 \tabularnewline
&Lasso with CV (2nd order poly)&-225.1&380.7&-728.4&245.7&-754.9&185.0&-231.7&122.5&703.7&44.5 \tabularnewline
&Ridge with CV (2nd order poly)&-1193.7&378.0&-1631.7&238.9&-1132.1&193.6&108.6&128.2&767.4&44.6 \tabularnewline
&Lasso with CV (10th order poly)&7612.9&4650.8&4713.5&7271.7&1131.3&5053.5&5091.8&4210.0&-4109.0&1325.8 \tabularnewline
&Ridge with CV (10th order poly)&16564.0&8040.5&8323.5&6357.0&5813.8&4655.8&-7529.8&3072.1&-5126.2&1713.9 \tabularnewline
&Random forest (low regularization)&444.2&360.6&38.3&244.1&-358.8&179.1&-420.4&119.7&-96.1&48.5 \tabularnewline
&Random forest (high regularization)&1056.8&340.6&-40.2&230.8&-335.9&171.1&-354.0&116.3&-159.7&43.5 \tabularnewline
&Gradient boosting (low regularization)&89.7&376.6&-58.3&253.4&-435.8&182.1&-390.4&116.4&8.5&42.7 \tabularnewline
&Gradient boosting (high regularization)&365.8&358.2&170.3&239.0&-193.0&172.8&-189.5&112.3&162.0&42.1 \tabularnewline
&Neural net&2357.6&335.2&2229.6&259.5&1965.1&198.8&1266.7&139.6&-601.3&46.5 \tabularnewline
&Stacking: CLS&656.2&1786.0&583.5&718.1&-393.0&500.7&-710.3&585.3&133.9&195.6 \tabularnewline
&Stacking: Average&2921.9&1220.8&2639.9&1126.1&318.6&1095.6&-656.9&526.5&94.0&110.3 \tabularnewline
&Stacking: OLS&2.2e7&1.9e7&-8671.2&9731.4&-5593.2&7804.4&971.5&3368.2&-204.8&405.2 \tabularnewline
&Stacking: Single-best&2892.1&1501.3&-442.5&347.7&-387.1&295.4&-311.5&506.8&-121.9&272.9 \tabularnewline
&Short-stacking: CLS&410.7&316.1&-76.2&215.5&-320.8&163.2&-219.0&107.8&162.7&42.0 \tabularnewline
&Short-stacking: Average&2921.9&1220.8&2639.9&1126.1&318.6&1095.6&-656.9&526.5&94.0&110.3 \tabularnewline
&Short-stacking: OLS&-130.7&287.7&-201.9&202.5&-322.2&155.3&-226.9&106.1&123.6&41.7 \tabularnewline
&Short-stacking: Single-best&-28.4&323.0&-363.6&221.3&-546.6&164.0&-320.3&110.4&71.7&42.6 \tabularnewline
&Pooled stacking: CLS&767.3&1131.7&942.5&577.0&-673.3&318.3&-734.7&567.8&209.8&63.7 \tabularnewline
&Pooled stacking: Average&2921.9&1220.8&2639.9&1126.1&318.6&1095.6&-656.9&526.5&94.0&110.3 \tabularnewline
&Pooled stacking: OLS&-1784.7&5455.8&-6585.3&4193.1&-897.4&1388.9&903.3&2480.1&234.5&124.9 \tabularnewline
&Pooled stacking: Single-best&1594.5&1414.5&-26.1&449.7&-557.8&366.5&-176.4&379.9&103.3&45.8 \tabularnewline


==> Simul/sim_Advantages/sim_output_folds2.tex <==
&OLS&49.9&793.8&0.95&&-6.8&281.2&0.95&&-2588.9&2576.5&0.58&&-2632.3&2611.5&0.\phantom{00} \tabularnewline
&PDS-Lasso&48.4&787.1&0.95&&-4.2&280.8&0.95&&-2598.7&2590.1&0.58&&-2631.6&2609.5&0.\phantom{00} \tabularnewline
&OLS&46.2&818.1&0.94&&-6.9&283.1&0.95&&-2613.0&2634.2&0.58&&-2635.4&2615.9&0.\phantom{00} \tabularnewline
&Lasso with CV (2nd order poly)&50.9&806.6&0.95&&-6.2&284.8&0.95&&703.7&1052.3&0.91&&718.5&712.8&0.60 \tabularnewline
&Ridge with CV (2nd order poly)&48.2&806.9&0.94&&-6.9&283.7&0.96&&767.4&1080.8&0.90&&729.3&724.0&0.60 \tabularnewline
&Lasso with CV (10th order poly)&248.1&1034.5&0.94&&55.9&285.9&0.95&&-4109.0&1799.9&0.90&&7.4&306.5&0.94 \tabularnewline
&Ridge with CV (10th order poly)&1230.1&1321.9&0.91&&31.6&283.0&0.96&&-5126.2&2215.7&0.89&&9.6&307.8&0.94 \tabularnewline
&Random forest (low regularization)&-74.7&1031.3&0.89&&-25.2&344.0&0.88&&-96.1&1037.1&0.90&&-37.5&328.0&0.87 \tabularnewline
&Random forest (high regularization)&69.1&891.2&0.94&&-23.5&287.6&0.93&&-159.7&904.4&0.94&&-4.2&280.4&0.95 \tabularnewline
&Gradient boosting (low regularization)&12.1&817.0&0.94&&-24.2&285.1&0.96&&8.5&866.0&0.94&&30.9&275.1&0.96 \tabularnewline
&Gradient boosting (high regularization)&114.8&823.8&0.94&&66.9&285.6&0.95&&162.0&857.2&0.94&&200.1&314.6&0.93 \tabularnewline
&Neural net&394.2&943.6&0.93&&9.1&287.5&0.94&&-601.3&1063.9&0.93&&-131.9&310.0&0.93 \tabularnewline
&Stacking: CLS&42.8&813.4&0.94&&-7.5&282.9&0.96&&133.9&1049.5&0.94&&37.8&271.0&0.95 \tabularnewline
&Stacking: Average&107.7&821.9&0.94&&-6.5&273.6&0.95&&94.0&1035.6&0.94&&72.3&289.3&0.96 \tabularnewline
&Stacking: OLS&-129.3&878.7&0.94&&-9.4&283.8&0.95&&-204.8&1184.9&0.94&&17.5&268.3&0.96 \tabularnewline
&Stacking: Single-best&43.7&819.8&0.94&&-8.6&281.4&0.95&&-121.9&976.2&0.94&&30.9&275.1&0.96 \tabularnewline
&Short-stacking: CLS&45.0&794.9&0.94&&-7.0&282.6&0.95&&162.7&865.1&0.94&&33.6&266.3&0.95 \tabularnewline
&Short-stacking: Average&107.7&821.9&0.94&&-6.5&273.6&0.95&&94.0&1035.6&0.94&&72.3&289.3&0.96 \tabularnewline
&Short-stacking: OLS&37.6&803.7&0.94&&-7.8&282.0&0.95&&123.6&863.5&0.94&&29.5&265.3&0.96 \tabularnewline
&Short-stacking: Single-best&44.4&817.8&0.94&&-8.3&281.9&0.95&&71.7&868.4&0.94&&30.9&275.1&0.96 \tabularnewline
&Pooled stacking: CLS&58.6&819.5&0.95&&-7.1&283.9&0.96&&209.8&921.0&0.94&&37.5&269.8&0.95 \tabularnewline
&Pooled stacking: Average&107.7&821.9&0.94&&-6.5&273.6&0.95&&94.0&1035.6&0.94&&72.3&289.3&0.96 \tabularnewline
&Pooled stacking: OLS&46.5&805.2&0.94&&-7.8&284.0&0.96&&234.5&1003.2&0.94&&30.6&266.3&0.96 \tabularnewline
&Pooled stacking: Single-best&46.9&823.5&0.94&&-8.3&282.6&0.95&&103.3&904.6&0.94&&30.9&275.1&0.96 \tabularnewline


==> Simul/sim_Advantages/sim_output_folds2_se.tex <==
&OLS&49.9&39.6&&-6.8&12.6&&-2588.9&46.5&&-2632.3&14.8 \tabularnewline
&PDS-Lasso&48.4&39.6&&-4.2&12.6&&-2598.7&46.5&&-2631.6&14.8 \tabularnewline
&OLS&46.2&39.7&&-6.9&12.6&&-2613.0&47.5&&-2635.4&14.8 \tabularnewline
&Lasso with CV (2nd order poly)&50.9&39.7&&-6.2&12.6&&703.7&44.5&&718.5&13.5 \tabularnewline
&Ridge with CV (2nd order poly)&48.2&39.9&&-6.9&12.6&&767.4&44.6&&729.3&13.5 \tabularnewline
&Lasso with CV (10th order poly)&248.1&266.6&&55.9&12.6&&-4109.0&1325.8&&7.4&22.5 \tabularnewline
&Ridge with CV (10th order poly)&1230.1&401.8&&31.6&12.6&&-5126.2&1713.9&&9.6&23.3 \tabularnewline
&Random forest (low regularization)&-74.7&48.6&&-25.2&16.0&&-96.1&48.5&&-37.5&15.4 \tabularnewline
&Random forest (high regularization)&69.1&41.7&&-23.5&13.2&&-159.7&43.5&&-4.2&13.0 \tabularnewline
&Gradient boosting (low regularization)&12.1&40.1&&-24.2&12.6&&8.5&42.7&&30.9&12.4 \tabularnewline
&Gradient boosting (high regularization)&114.8&39.8&&66.9&12.5&&162.0&42.1&&200.1&12.6 \tabularnewline
&Neural net&394.2&43.1&&9.1&13.6&&-601.3&46.5&&-131.9&14.3 \tabularnewline
&Stacking: CLS&42.8&40.2&&-7.5&12.6&&133.9&195.6&&37.8&12.4 \tabularnewline
&Stacking: Average&107.7&51.2&&-6.5&12.6&&94.0&110.3&&72.3&12.7 \tabularnewline
&Stacking: OLS&-129.3&96.2&&-9.4&14.9&&-204.8&405.2&&17.5&17.8 \tabularnewline
&Stacking: Single-best&43.7&39.9&&-8.6&12.6&&-121.9&272.9&&30.9&12.4 \tabularnewline
&Short-stacking: CLS&45.0&39.7&&-7.0&12.6&&162.7&42.0&&33.6&12.4 \tabularnewline
&Short-stacking: Average&107.7&51.2&&-6.5&12.6&&94.0&110.3&&72.3&12.7 \tabularnewline
&Short-stacking: OLS&37.6&39.6&&-7.8&12.6&&123.6&41.7&&29.5&12.3 \tabularnewline
&Short-stacking: Single-best&44.4&39.7&&-8.3&12.6&&71.7&42.6&&30.9&12.4 \tabularnewline
&Pooled stacking: CLS&58.6&41.4&&-7.1&12.6&&209.8&63.7&&37.5&12.4 \tabularnewline
&Pooled stacking: Average&107.7&51.2&&-6.5&12.6&&94.0&110.3&&72.3&12.7 \tabularnewline
&Pooled stacking: OLS&46.5&47.8&&-7.8&12.6&&234.5&124.9&&30.6&12.3 \tabularnewline
&Pooled stacking: Single-best&46.9&39.7&&-8.3&12.6&&103.3&45.8&&30.9&12.4 \tabularnewline


==> Simul/sim_Advantages/sim_small_bias_wide_folds10.tex <==
&OLS&230.4&-28.4&9.7&11.7&78.3&&-2339.8&-2208.9&-2332.7&-2440.2&-2586.2 \tabularnewline
&PDS-Lasso&-714.3&-739.5&-367.9&-76.3&78.8&&-2281.9&-2740.9&-2789.1&-2716.2&-2597.3 \tabularnewline
&OLS&179.4&-85.1&2.5&7.9&77.8&&-2864.1&-2607.8&-2479.6&-2526.7&-2606.5 \tabularnewline
&Lasso with CV (2nd order poly)&357.0&-38.9&3.4&9.1&77.5&&-1048.1&-730.3&243.2&467.6&783.4 \tabularnewline
&Ridge with CV (2nd order poly)&334.6&6.4&10.8&-9.9&77.5&&-1730.2&-1127.8&481.5&833.2&806.7 \tabularnewline
&Lasso with CV (10th order poly)&-4864.6&754.7&-476.8&-547.1&141.0&&22248.8&-2907.1&1598.1&4485.9&185.6 \tabularnewline
&Ridge with CV (10th order poly)&-14274.3&1038.4&1596.6&1442.5&449.8&&24105.0&2351.6&-5341.5&-602.5&2873.4 \tabularnewline
&Random forest (low regularization)&328.1&-112.2&-148.4&-69.6&-41.8&&-84.4&18.2&-5.4&-89.8&-63.6 \tabularnewline
&Random forest (high regularization)&1086.7&255.6&206.3&128.5&68.4&&-159.0&-37.4&99.8&-77.1&-78.1 \tabularnewline
&Gradient boosting (low regularization)&171.1&-280.4&-149.1&-60.3&44.3&&-281.5&-32.4&-11.1&34.1&64.6 \tabularnewline
&Gradient boosting (high regularization)&389.4&-77.4&65.0&75.2&139.1&&-89.7&208.6&179.2&182.9&218.2 \tabularnewline
&Neural net&3887.7&3926.3&3504.2&1874.9&212.1&&1839.2&2045.7&1735.2&209.6&-472.8 \tabularnewline
&Stacking: CLS&-1150.3&-84.3&28.2&47.1&73.1&&11936.9&-1198.8&803.6&915.4&437.8 \tabularnewline
&Stacking: Average&-3471.2&195.7&-71.7&368.6&86.3&&7161.2&498.4&-368.8&765.1&451.8 \tabularnewline
&Stacking: OLS&4.2e6&-1040.5&-2085.4&-365.2&32.8&&-2.7e7&-3391.9&3033.6&6271.2&608.4 \tabularnewline
&Stacking: Single-best&-5.0&-212.2&-57.8&-27.6&68.2&&3472.5&-385.1&687.0&542.5&154.1 \tabularnewline
&Short-stacking: CLS&322.3&-54.8&51.6&25.1&73.2&&-278.6&-117.9&88.3&188.6&157.7 \tabularnewline
&Short-stacking: Average&-3471.2&195.7&-71.7&368.6&86.3&&7161.2&498.4&-368.8&765.1&451.8 \tabularnewline
&Short-stacking: OLS&-214.9&-278.5&-100.4&-41.0&70.7&&-524.0&-209.4&16.5&88.7&126.1 \tabularnewline
&Short-stacking: Single-best&189.1&-91.4&0.7&3.1&75.9&&-602.8&-363.9&51.5&196.2&66.9 \tabularnewline
&Pooled stacking: CLS&465.6&39.7&89.6&18.0&73.7&&-382.2&-319.7&-73.3&143.9&179.9 \tabularnewline
&Pooled stacking: Average&-3471.2&195.7&-71.7&368.6&86.3&&7161.2&498.4&-368.8&765.1&451.8 \tabularnewline
&Pooled stacking: OLS&326.6&-97.4&-68.3&-23.2&72.6&&-217.6&-231.1&-223.3&-23.4&152.0 \tabularnewline
&Pooled stacking: Single-best&150.8&-93.1&-11.6&8.3&76.6&&-679.0&-316.5&-52.0&159.4&68.2 \tabularnewline


==> Simul/sim_Advantages/sim_small_bias_wide_folds2.tex <==
&OLS&-67.4&190.0&-24.4&155.3&49.9&&-1890.5&-2398.9&-2645.8&-2793.8&-2588.9 \tabularnewline
&PDS-Lasso&-1126.6&-577.4&-431.5&66.8&48.4&&-2001.6&-2953.3&-3105.9&-3078.5&-2598.7 \tabularnewline
&OLS&-53.0&236.6&-22.0&186.4&46.2&&-2466.6&-2861.0&-2993.2&-2886.0&-2613.0 \tabularnewline
&Lasso with CV (2nd order poly)&345.5&262.7&5.7&193.5&50.9&&-225.1&-728.4&-754.9&-231.7&703.7 \tabularnewline
&Ridge with CV (2nd order poly)&313.7&293.8&120.1&213.8&48.2&&-1193.7&-1631.7&-1132.1&108.6&767.4 \tabularnewline
&Lasso with CV (10th order poly)&25276.6&-1632.0&742.4&1470.1&248.1&&7612.9&4713.5&1131.3&5091.8&-4109.0 \tabularnewline
&Ridge with CV (10th order poly)&7927.1&-267.5&6359.4&2776.4&1230.1&&16564.0&8323.5&5813.8&-7529.8&-5126.2 \tabularnewline
&Random forest (low regularization)&240.3&89.3&-255.9&22.4&-74.7&&444.2&38.3&-358.8&-420.4&-96.1 \tabularnewline
&Random forest (high regularization)&2159.2&999.1&332.8&355.0&69.1&&1056.8&-40.2&-335.9&-354.0&-159.7 \tabularnewline
&Gradient boosting (low regularization)&-167.8&-85.0&-294.2&89.2&12.1&&89.7&-58.3&-435.8&-390.4&8.5 \tabularnewline
&Gradient boosting (high regularization)&129.5&169.1&-64.4&252.6&114.8&&365.8&170.3&-193.0&-189.5&162.0 \tabularnewline
&Neural net&4241.3&4422.9&4260.5&3536.2&394.2&&2357.6&2229.6&1965.1&1266.7&-601.3 \tabularnewline
&Stacking: CLS&6329.4&-66.9&-21.5&261.0&42.8&&656.2&583.5&-393.0&-710.3&133.9 \tabularnewline
&Stacking: Average&-972.6&1796.8&254.6&815.2&107.7&&2921.9&2639.9&318.6&-656.9&94.0 \tabularnewline
&Stacking: OLS&-10699.3&3.8e7&-63.3&-1043.6&-129.3&&2.2e7&-8671.2&-5593.2&971.5&-204.8 \tabularnewline
&Stacking: Single-best&5893.9&73.8&-158.5&115.1&43.7&&2892.1&-442.5&-387.1&-311.5&-121.9 \tabularnewline
&Short-stacking: CLS&389.3&314.6&9.9&218.4&45.0&&410.7&-76.2&-320.8&-219.0&162.7 \tabularnewline
&Short-stacking: Average&-972.6&1796.8&254.6&815.2&107.7&&2921.9&2639.9&318.6&-656.9&94.0 \tabularnewline
&Short-stacking: OLS&-207.9&84.7&-113.2&124.9&37.6&&-130.7&-201.9&-322.2&-226.9&123.6 \tabularnewline
&Short-stacking: Single-best&241.8&209.2&-37.5&178.8&44.4&&-28.4&-363.6&-546.6&-320.3&71.7 \tabularnewline
&Pooled stacking: CLS&-22063.1&378.9&-141.5&230.4&58.6&&767.3&942.5&-673.3&-734.7&209.8 \tabularnewline
&Pooled stacking: Average&-972.6&1796.8&254.6&815.2&107.7&&2921.9&2639.9&318.6&-656.9&94.0 \tabularnewline
&Pooled stacking: OLS&-26101.3&-2324.4&-1641.0&-79.0&46.5&&-1784.7&-6585.3&-897.4&903.3&234.5 \tabularnewline
&Pooled stacking: Single-best&12247.4&122.1&-88.2&156.7&46.9&&1594.5&-26.1&-557.8&-176.4&103.3 \tabularnewline


==> Simul/sim_Advantages/sim_small_cover_wide_folds10.tex <==
&OLS&0.95&0.95&0.95&0.94&0.95&&0.92&0.95&0.94&0.92&0.59 \tabularnewline
&PDS-Lasso&0.96&0.95&0.94&0.94&0.95&&0.92&0.95&0.93&0.91&0.59 \tabularnewline
&OLS&0.95&0.95&0.94&0.94&0.94&&0.93&0.95&0.94&0.91&0.59 \tabularnewline
&Lasso with CV (2nd order poly)&0.95&0.95&0.94&0.93&0.94&&0.94&0.95&0.96&0.94&0.90 \tabularnewline
&Ridge with CV (2nd order poly)&0.96&0.95&0.94&0.94&0.94&&0.94&0.96&0.96&0.94&0.90 \tabularnewline
&Lasso with CV (10th order poly)&0.90&0.92&0.91&0.93&0.94&&0.87&0.85&0.86&0.89&0.95 \tabularnewline
&Ridge with CV (10th order poly)&0.82&0.87&0.88&0.88&0.95&&0.78&0.83&0.84&0.87&0.95 \tabularnewline
&Random forest (low regularization)&0.92&0.93&0.92&0.91&0.91&&0.92&0.93&0.94&0.93&0.90 \tabularnewline
&Random forest (high regularization)&0.95&0.94&0.95&0.94&0.95&&0.94&0.95&0.96&0.95&0.94 \tabularnewline
&Gradient boosting (low regularization)&0.92&0.93&0.93&0.94&0.95&&0.92&0.93&0.95&0.95&0.95 \tabularnewline
&Gradient boosting (high regularization)&0.94&0.95&0.94&0.94&0.95&&0.93&0.94&0.97&0.95&0.94 \tabularnewline
&Neural net&0.94&0.92&0.90&0.90&0.95&&0.94&0.95&0.95&0.97&0.94 \tabularnewline
&Stacking: CLS&0.94&0.95&0.94&0.93&0.95&&0.92&0.94&0.94&0.94&0.95 \tabularnewline
&Stacking: Average&0.94&0.95&0.94&0.94&0.95&&0.90&0.93&0.95&0.95&0.95 \tabularnewline
&Stacking: OLS&0.85&0.89&0.89&0.90&0.93&&0.82&0.86&0.89&0.92&0.93 \tabularnewline
&Stacking: Single-best&0.94&0.94&0.95&0.94&0.95&&0.94&0.94&0.95&0.95&0.94 \tabularnewline
&Short-stacking: CLS&0.95&0.95&0.94&0.94&0.94&&0.94&0.96&0.96&0.95&0.94 \tabularnewline
&Short-stacking: Average&0.94&0.95&0.94&0.94&0.95&&0.90&0.93&0.95&0.95&0.95 \tabularnewline
&Short-stacking: OLS&0.95&0.94&0.95&0.94&0.95&&0.94&0.95&0.95&0.95&0.94 \tabularnewline
&Short-stacking: Single-best&0.95&0.95&0.94&0.94&0.94&&0.93&0.96&0.96&0.96&0.95 \tabularnewline
&Pooled stacking: CLS&0.95&0.95&0.94&0.94&0.94&&0.94&0.95&0.96&0.95&0.94 \tabularnewline
&Pooled stacking: Average&0.94&0.95&0.94&0.94&0.95&&0.90&0.93&0.95&0.95&0.95 \tabularnewline
&Pooled stacking: OLS&0.95&0.95&0.94&0.94&0.94&&0.94&0.96&0.96&0.95&0.94 \tabularnewline
&Pooled stacking: Single-best&0.95&0.95&0.94&0.94&0.94&&0.94&0.95&0.95&0.95&0.95 \tabularnewline


==> Simul/sim_Advantages/sim_small_cover_wide_folds2.tex <==
&OLS&0.95&0.94&0.95&0.95&0.95&&0.95&0.94&0.92&0.89&0.58 \tabularnewline
&PDS-Lasso&0.94&0.94&0.94&0.95&0.95&&0.94&0.93&0.92&0.89&0.58 \tabularnewline
&OLS&0.90&0.91&0.93&0.95&0.94&&0.89&0.91&0.90&0.89&0.58 \tabularnewline
&Lasso with CV (2nd order poly)&0.94&0.93&0.94&0.95&0.95&&0.93&0.94&0.92&0.94&0.91 \tabularnewline
&Ridge with CV (2nd order poly)&0.94&0.93&0.94&0.95&0.94&&0.93&0.94&0.92&0.93&0.90 \tabularnewline
&Lasso with CV (10th order poly)&0.88&0.86&0.89&0.91&0.94&&0.84&0.81&0.81&0.82&0.90 \tabularnewline
&Ridge with CV (10th order poly)&0.71&0.76&0.83&0.83&0.91&&0.72&0.72&0.79&0.81&0.89 \tabularnewline
&Random forest (low regularization)&0.92&0.90&0.91&0.91&0.89&&0.91&0.92&0.91&0.91&0.90 \tabularnewline
&Random forest (high regularization)&0.94&0.93&0.94&0.94&0.94&&0.94&0.94&0.94&0.93&0.94 \tabularnewline
&Gradient boosting (low regularization)&0.92&0.89&0.92&0.94&0.94&&0.89&0.92&0.92&0.94&0.94 \tabularnewline
&Gradient boosting (high regularization)&0.93&0.93&0.93&0.94&0.94&&0.91&0.93&0.93&0.94&0.94 \tabularnewline
&Neural net&0.90&0.83&0.80&0.79&0.93&&0.91&0.90&0.88&0.88&0.93 \tabularnewline
&Stacking: CLS&0.90&0.90&0.93&0.94&0.94&&0.90&0.92&0.93&0.93&0.94 \tabularnewline
&Stacking: Average&0.90&0.91&0.93&0.93&0.94&&0.89&0.90&0.91&0.92&0.94 \tabularnewline
&Stacking: OLS&0.71&0.78&0.88&0.90&0.94&&0.68&0.76&0.83&0.87&0.94 \tabularnewline
&Stacking: Single-best&0.91&0.91&0.93&0.94&0.94&&0.92&0.93&0.93&0.93&0.94 \tabularnewline
&Short-stacking: CLS&0.94&0.93&0.94&0.95&0.94&&0.93&0.94&0.93&0.94&0.94 \tabularnewline
&Short-stacking: Average&0.90&0.91&0.93&0.93&0.94&&0.89&0.90&0.91&0.92&0.94 \tabularnewline
&Short-stacking: OLS&0.95&0.94&0.94&0.94&0.94&&0.94&0.94&0.93&0.95&0.94 \tabularnewline
&Short-stacking: Single-best&0.94&0.93&0.94&0.94&0.94&&0.94&0.94&0.94&0.95&0.94 \tabularnewline
&Pooled stacking: CLS&0.93&0.90&0.93&0.94&0.95&&0.92&0.94&0.93&0.95&0.94 \tabularnewline
&Pooled stacking: Average&0.90&0.91&0.93&0.93&0.94&&0.89&0.90&0.91&0.92&0.94 \tabularnewline
&Pooled stacking: OLS&0.88&0.89&0.92&0.93&0.94&&0.85&0.90&0.90&0.93&0.94 \tabularnewline
&Pooled stacking: Single-best&0.94&0.92&0.93&0.95&0.94&&0.94&0.95&0.94&0.95&0.94 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_grad_large_nopooled.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (2nd order poly)&0.\phantom{000}&0.036&&0.\phantom{000}&0.026 \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.001&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.036&&0.\phantom{000}&0.024 \tabularnewline
Random forest (low regularization)&0.153&0.003&&0.180&0.001 \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.060&&0.\phantom{000}&0.071 \tabularnewline
Gradient boosting (low regularization)&0.845&0.853&&0.819&0.871 \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.001&0.012&&0.001&0.007 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_grad_nopooled.tex <==
OLS&0.011&0.015&&0.004&0.007 \tabularnewline
Lasso with CV (2nd order poly)&0.035&0.057&&0.019&0.039 \tabularnewline
Ridge with CV (2nd order poly)&0.161&0.229&&0.114&0.237 \tabularnewline
Lasso with CV (10th order poly)&0.053&0.080&&0.048&0.062 \tabularnewline
Ridge with CV (10th order poly)&0.071&0.064&&0.059&0.056 \tabularnewline
Random forest (low regularization)&0.045&0.011&&0.043&0.005 \tabularnewline
Random forest (high regularization)&0.019&0.069&&0.012&0.065 \tabularnewline
Gradient boosting (low regularization)&0.521&0.233&&0.632&0.339 \tabularnewline
Gradient boosting (high regularization)&0.014&0.191&&0.004&0.139 \tabularnewline
Neural net&0.071&0.051&&0.064&0.049 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_ols_large_nopooled.tex <==
OLS&0.770&0.325&&0.769&0.291 \tabularnewline
Lasso with CV (2nd order poly)&0.066&0.026&&0.068&0.013 \tabularnewline
Ridge with CV (2nd order poly)&0.074&0.041&&0.094&0.049 \tabularnewline
Lasso with CV (10th order poly)&0.015&0.207&&0.011&0.198 \tabularnewline
Ridge with CV (10th order poly)&0.023&0.111&&0.019&0.129 \tabularnewline
Random forest (low regularization)&0.003&0.003&&0.002&0.002 \tabularnewline
Random forest (high regularization)&0.006&0.009&&0.005&0.006 \tabularnewline
Gradient boosting (low regularization)&0.019&0.160&&0.013&0.186 \tabularnewline
Gradient boosting (high regularization)&0.004&0.008&&0.003&0.003 \tabularnewline
Neural net&0.019&0.110&&0.016&0.122 \tabularnewline


==> Simul/sim_Advantages/sweights_nnls1_ols_nopooled.tex <==
OLS&0.668&0.501&&0.692&0.492 \tabularnewline
Lasso with CV (2nd order poly)&0.105&0.144&&0.118&0.130 \tabularnewline
Ridge with CV (2nd order poly)&0.068&0.054&&0.068&0.063 \tabularnewline
Lasso with CV (10th order poly)&0.027&0.073&&0.020&0.085 \tabularnewline
Ridge with CV (10th order poly)&0.033&0.043&&0.024&0.057 \tabularnewline
Random forest (low regularization)&0.013&0.011&&0.009&0.008 \tabularnewline
Random forest (high regularization)&0.017&0.024&&0.013&0.024 \tabularnewline
Gradient boosting (low regularization)&0.030&0.043&&0.020&0.040 \tabularnewline
Gradient boosting (high regularization)&0.020&0.060&&0.018&0.060 \tabularnewline
Neural net&0.019&0.049&&0.018&0.043 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_grad_large_nopooled.tex <==
OLS&--0.015&0.009&&0.\phantom{000}&0.009 \tabularnewline
Lasso with CV (2nd order poly)&0.089&--0.806&&--0.026&--0.721 \tabularnewline
Ridge with CV (2nd order poly)&--0.171&0.792&&--0.053&0.696 \tabularnewline
Lasso with CV (10th order poly)&0.285&--0.247&&0.358&--0.325 \tabularnewline
Ridge with CV (10th order poly)&--0.338&0.320&&--0.425&0.383 \tabularnewline
Random forest (low regularization)&0.142&--0.011&&0.168&--0.013 \tabularnewline
Random forest (high regularization)&--0.111&0.069&&--0.125&0.079 \tabularnewline
Gradient boosting (low regularization)&2.368&1.233&&2.353&1.332 \tabularnewline
Gradient boosting (high regularization)&--1.443&--0.403&&--1.424&--0.498 \tabularnewline
Neural net&--45.762&0.030&&0.066&0.040 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_grad_nopooled.tex <==
OLS&0.013&0.050&&--0.048&0.022 \tabularnewline
Lasso with CV (2nd order poly)&--0.118&--0.319&&0.033&--0.347 \tabularnewline
Ridge with CV (2nd order poly)&0.365&0.528&&0.146&0.548 \tabularnewline
Lasso with CV (10th order poly)&--0.014&0.126&&0.091&0.088 \tabularnewline
Ridge with CV (10th order poly)&0.060&0.028&&--0.011&0.055 \tabularnewline
Random forest (low regularization)&0.052&--0.016&&0.057&--0.016 \tabularnewline
Random forest (high regularization)&--0.098&0.059&&--0.110&0.064 \tabularnewline
Gradient boosting (low regularization)&1.096&0.029&&1.358&0.159 \tabularnewline
Gradient boosting (high regularization)&--0.531&0.526&&--0.716&0.426 \tabularnewline
Neural net&--72.340&0.027&&0.120&0.054 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_ols_large_nopooled.tex <==
OLS&1.292&0.935&&1.008&0.677 \tabularnewline
Lasso with CV (2nd order poly)&--0.103&--0.497&&0.033&--0.398 \tabularnewline
Ridge with CV (2nd order poly)&--0.170&--0.053&&--0.044&0.056 \tabularnewline
Lasso with CV (10th order poly)&0.065&0.407&&0.009&0.335 \tabularnewline
Ridge with CV (10th order poly)&--0.071&--0.118&&--0.003&--0.034 \tabularnewline
Random forest (low regularization)&--0.000&--0.001&&0.\phantom{000}&--0.001 \tabularnewline
Random forest (high regularization)&--0.001&--0.002&&--0.000&--0.001 \tabularnewline
Gradient boosting (low regularization)&--0.034&0.158&&--0.020&0.224 \tabularnewline
Gradient boosting (high regularization)&0.034&0.072&&0.022&0.020 \tabularnewline
Neural net&--12.267&0.110&&--0.003&0.133 \tabularnewline


==> Simul/sim_Advantages/sweights_ols_ols_nopooled.tex <==
OLS&1.161&0.932&&0.923&0.686 \tabularnewline
Lasso with CV (2nd order poly)&0.011&0.034&&0.154&0.079 \tabularnewline
Ridge with CV (2nd order poly)&--0.157&--0.187&&--0.080&--0.080 \tabularnewline
Lasso with CV (10th order poly)&--0.046&0.076&&--0.041&0.122 \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&--0.006&&0.017&0.022 \tabularnewline
Random forest (low regularization)&0.001&--0.005&&0.003&--0.006 \tabularnewline
Random forest (high regularization)&--0.014&--0.006&&--0.011&0.008 \tabularnewline
Gradient boosting (low regularization)&--0.060&--0.108&&--0.039&--0.094 \tabularnewline
Gradient boosting (high regularization)&0.096&0.260&&0.076&0.257 \tabularnewline
Neural net&--195.245&0.009&&0.004&0.033 \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_grad_large_nopooled.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (2nd order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&1.\phantom{000}&1.\phantom{000}&&1.\phantom{000}&1.\phantom{000} \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_grad_nopooled.tex <==
OLS&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Lasso with CV (2nd order poly)&0.093&0.149&&0.054&0.081 \tabularnewline
Ridge with CV (2nd order poly)&0.132&0.124&&0.058&0.093 \tabularnewline
Lasso with CV (10th order poly)&0.072&0.058&&0.039&0.026 \tabularnewline
Ridge with CV (10th order poly)&0.019&0.041&&0.005&0.037 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.002&0.001&&0.002&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.673&0.357&&0.832&0.623 \tabularnewline
Gradient boosting (high regularization)&0.009&0.268&&0.008&0.140 \tabularnewline
Neural net&0.002&0.002&&0.002&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_ols_large_nopooled.tex <==
OLS&0.895&0.292&&0.880&0.181 \tabularnewline
Lasso with CV (2nd order poly)&0.087&0.093&&0.078&0.059 \tabularnewline
Ridge with CV (2nd order poly)&0.018&0.016&&0.042&0.017 \tabularnewline
Lasso with CV (10th order poly)&0.\phantom{000}&0.186&&0.\phantom{000}&0.151 \tabularnewline
Ridge with CV (10th order poly)&0.\phantom{000}&0.410&&0.\phantom{000}&0.591 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.\phantom{000}&0.002&&0.\phantom{000}&0.001 \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_Advantages/sweights_singlebest_ols_nopooled.tex <==
OLS&0.812&0.645&&0.821&0.650 \tabularnewline
Lasso with CV (2nd order poly)&0.163&0.274&&0.150&0.266 \tabularnewline
Ridge with CV (2nd order poly)&0.021&0.016&&0.028&0.027 \tabularnewline
Lasso with CV (10th order poly)&0.002&0.048&&0.001&0.034 \tabularnewline
Ridge with CV (10th order poly)&0.002&0.010&&0.\phantom{000}&0.023 \tabularnewline
Random forest (low regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Random forest (high regularization)&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (low regularization)&0.\phantom{000}&0.003&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Gradient boosting (high regularization)&0.\phantom{000}&0.003&&0.\phantom{000}&0.\phantom{000} \tabularnewline
Neural net&0.\phantom{000}&0.\phantom{000}&&0.\phantom{000}&0.\phantom{000} \tabularnewline


==> Simul/sim_WZ/bias_ddml_candidate_f2.tex <==
&OLS&-509.4&440.4&-643.7&-270.5&243.3&192 \tabularnewline
&Lasso with CV (TWI)&7184.1&5485.8&3408.9&2998&2509.6&1848 \tabularnewline
&Ridge with CV (TWI)&4659.4&3674.3&1888.4&1649.9&1433.4&1189.6 \tabularnewline
&Lasso with CV (QSI)&911.3&191.9&-874.5&-628.5&-207.1&-286.3 \tabularnewline
&Ridge with CV (QSI)&213.3&269.4&-533.9&-304.8&154&49.3 \tabularnewline
&Random forest (low regularization)&1689.7&1136.3&-88.2&311.6&652&455.5 \tabularnewline
&Random forest (high regularization)&14334.3&8404.1&4923.6&3493.2&2704.6&1982.3 \tabularnewline
&Gradient boosting (low regularization)&-391.8&32.1&-668.6&-185&373.4&314.6 \tabularnewline
&Gradient boosting (high regularization)&-95.5&301.8&-370.1&85.5&615.4&519.8 \tabularnewline
&Neural net&9433.7&9725&7407.1&7627.3&6552.1&5595.1 \tabularnewline


==> Simul/sim_WZ/bias_olspds_f2.tex <==
&OLS QSI&-2532.3&-1311.4&-1421.9&-961.6&-399&-282.2 \tabularnewline
&OLS TWI&-2100.3&-448&-936.5&-531.8&23.1&244.7 \tabularnewline
&Post double Lasso QSI c=0.5&-154.7&-120.1&-1019.8&-628.9&-50.5&-161.7 \tabularnewline
&Post double Lasso QSI c=1&-600.6&-1053&-1576.5&-1079&-485.1&-424.9 \tabularnewline
&Post double Lasso QSI c=1.5&7836.3&1064&-2253.4&-2434.8&-1644.7&-1698.3 \tabularnewline
&Post double Lasso TWI c=0.5&2868.8&2792.2&1635.4&1595.6&1767.6&1460.7 \tabularnewline
&Post double Lasso TWI c=1&5201.7&3964.3&2742&2328.1&2174.8&1975.8 \tabularnewline
&Post double Lasso TWI c=1.5&13619.4&9399.4&5610&4277&4150.8&3065.3 \tabularnewline


==> Simul/sim_WZ/fullsample_meta.tex <==
&Pooled stacking: CLS&5822.695 \tabularnewline
&Pooled stacking: Single-best&5717.825 \tabularnewline
&Short-stacking: CLS&5803.858 \tabularnewline
&Short-stacking: Single-best&5697.312 \tabularnewline
&Stacking: CLS&5767.291 \tabularnewline
&Stacking: Single-best&5661.027 \tabularnewline


==> Simul/sim_WZ/psw_d_nnls1_folds10.tex <==
&OLS&.129&.207&.257&.279&.252&.221&.007 \tabularnewline
&Neural net&.013&.013&.012&.012&.01&.013&.043 \tabularnewline
&Lasso with CV (TWI)&.028&.017&.014&.01&.008&.007&.104 \tabularnewline
&Ridge with CV (TWI)&.037&.011&.005&.008&.008&.008&.001 \tabularnewline
&Lasso with CV (QSI)&.129&.205&.261&.281&.304&.296&.452 \tabularnewline
&Ridge with CV (QSI)&.239&.169&.085&.046&.049&.058&.011 \tabularnewline
&Random forest (low regularization)&.106&.117&.133&.168&.221&.271&.007 \tabularnewline
&Random forest (high regularization)&.257&.189&.155&.133&.087&.066&.131 \tabularnewline
&Gradient boosting (low regularization)&.021&.025&.032&.028&.029&.036&.241 \tabularnewline
&Gradient boosting (high regularization)&.041&.047&.048&.035&.033&.024&.003 \tabularnewline


==> Simul/sim_WZ/psw_d_nnls1_folds2.tex <==
&OLS&.078&.142&.189&.226&.261&.279&.143 \tabularnewline
&Neural net&.041&.031&.036&.033&.03&.028&.043 \tabularnewline
&Lasso with CV (TWI)&.059&.029&.016&.017&.012&.009&.028 \tabularnewline
&Ridge with CV (TWI)&.075&.033&.016&.011&.008&.006&.002 \tabularnewline
&Lasso with CV (QSI)&.128&.147&.202&.231&.27&.273&.424 \tabularnewline
&Ridge with CV (QSI)&.176&.227&.178&.132&.061&.044&.005 \tabularnewline
&Random forest (low regularization)&.111&.093&.1&.108&.14&.174&.01 \tabularnewline
&Random forest (high regularization)&.258&.22&.178&.158&.14&.117&.173 \tabularnewline
&Gradient boosting (low regularization)&.026&.028&.032&.033&.033&.035&.169 \tabularnewline
&Gradient boosting (high regularization)&.05&.051&.052&.051&.044&.035&.003 \tabularnewline


==> Simul/sim_WZ/psw_d_singlebest_folds10.tex <==
&OLS&.015&.076&.135&.184&.174&.128&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.023&.009&.007&.002&0&0&0 \tabularnewline
&Ridge with CV (TWI)&.087&.008&.002&.006&.001&.001&0 \tabularnewline
&Lasso with CV (QSI)&.19&.313&.355&.335&.32&.212&.95 \tabularnewline
&Ridge with CV (QSI)&.299&.175&.034&.011&.025&.026&0 \tabularnewline
&Random forest (low regularization)&.084&.018&.005&.002&0&0&0 \tabularnewline
&Random forest (high regularization)&.256&.309&.344&.376&.396&.555&0 \tabularnewline
&Gradient boosting (low regularization)&.001&.002&.006&.011&.038&.065&.05 \tabularnewline
&Gradient boosting (high regularization)&.044&.09&.112&.073&.044&.012&0 \tabularnewline


==> Simul/sim_WZ/psw_d_singlebest_folds2.tex <==
&OLS&.001&.019&.056&.084&.152&.188&.237 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.055&.02&.009&.008&.004&.002&0 \tabularnewline
&Ridge with CV (TWI)&.213&.074&.012&.005&.002&.002&0 \tabularnewline
&Lasso with CV (QSI)&.174&.222&.322&.362&.358&.299&.586 \tabularnewline
&Ridge with CV (QSI)&.158&.3&.197&.094&.011&.009&0 \tabularnewline
&Random forest (low regularization)&.169&.051&.021&.005&.001&0&0 \tabularnewline
&Random forest (high regularization)&.192&.246&.284&.323&.35&.39&.011 \tabularnewline
&Gradient boosting (low regularization)&.001&.002&.001&.002&.01&.026&.166 \tabularnewline
&Gradient boosting (high regularization)&.037&.065&.098&.115&.111&.082&0 \tabularnewline


==> Simul/sim_WZ/psw_y_nnls1_folds10.tex <==
&OLS&.151&.147&.12&.093&.048&.026&0 \tabularnewline
&Neural net&.232&.238&.248&.191&.117&.039&.07 \tabularnewline
&Lasso with CV (TWI)&.023&.017&.02&.021&.021&.025&.072 \tabularnewline
&Ridge with CV (TWI)&.033&.034&.035&.025&.016&.013&.061 \tabularnewline
&Lasso with CV (QSI)&.179&.204&.193&.209&.229&.259&.607 \tabularnewline
&Ridge with CV (QSI)&.167&.21&.242&.308&.38&.416&.175 \tabularnewline
&Random forest (low regularization)&.095&.076&.087&.103&.142&.181&.008 \tabularnewline
&Random forest (high regularization)&.085&.039&.019&.017&.023&.022&.003 \tabularnewline
&Gradient boosting (low regularization)&.02&.022&.027&.025&.023&.017&.002 \tabularnewline
&Gradient boosting (high regularization)&.017&.012&.01&.007&.001&.001&.003 \tabularnewline


==> Simul/sim_WZ/psw_y_nnls1_folds2.tex <==
&OLS&.124&.168&.177&.16&.122&.086&0 \tabularnewline
&Neural net&.123&.084&.097&.087&.095&.123&.034 \tabularnewline
&Lasso with CV (TWI)&.038&.033&.026&.025&.021&.022&.133 \tabularnewline
&Ridge with CV (TWI)&.049&.037&.04&.035&.028&.019&.003 \tabularnewline
&Lasso with CV (QSI)&.184&.234&.263&.271&.263&.25&.501 \tabularnewline
&Ridge with CV (QSI)&.189&.217&.212&.259&.305&.334&.304 \tabularnewline
&Random forest (low regularization)&.165&.095&.087&.085&.101&.112&.022 \tabularnewline
&Random forest (high regularization)&.072&.081&.05&.033&.021&.017&.003 \tabularnewline
&Gradient boosting (low regularization)&.028&.029&.032&.032&.035&.03&.001 \tabularnewline
&Gradient boosting (high regularization)&.029&.021&.017&.014&.009&.006&0 \tabularnewline


==> Simul/sim_WZ/psw_y_singlebest_folds10.tex <==
&OLS&.114&.141&.095&.039&.006&.001&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.01&.006&.004&.004&.004&.011&0 \tabularnewline
&Ridge with CV (TWI)&.053&.062&.081&.072&.042&.019&0 \tabularnewline
&Lasso with CV (QSI)&.293&.375&.355&.347&.331&.344&1 \tabularnewline
&Ridge with CV (QSI)&.271&.333&.4&.488&.574&.577&0 \tabularnewline
&Random forest (low regularization)&.213&.06&.04&.033&.029&.023&0 \tabularnewline
&Random forest (high regularization)&.026&.005&0&0&0&0&0 \tabularnewline
&Gradient boosting (low regularization)&.004&.008&.02&.015&.015&.025&0 \tabularnewline
&Gradient boosting (high regularization)&.015&.01&.005&.001&0&0&0 \tabularnewline


==> Simul/sim_WZ/psw_y_singlebest_folds2.tex <==
&OLS&.019&.104&.136&.098&.048&.014&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.017&.014&.008&.007&.004&.006&.002 \tabularnewline
&Ridge with CV (TWI)&.094&.059&.056&.057&.06&.042&0 \tabularnewline
&Lasso with CV (QSI)&.22&.322&.4&.407&.391&.371&.762 \tabularnewline
&Ridge with CV (QSI)&.244&.299&.293&.356&.447&.521&.237 \tabularnewline
&Random forest (low regularization)&.367&.16&.076&.048&.029&.023&0 \tabularnewline
&Random forest (high regularization)&.009&.013&.006&.002&0&0&0 \tabularnewline
&Gradient boosting (low regularization)&.008&.007&.009&.014&.017&.02&0 \tabularnewline
&Gradient boosting (high regularization)&.023&.023&.016&.011&.005&.002&0 \tabularnewline


==> Simul/sim_WZ/ssw_d_nnls1_folds2.tex <==
&OLS&.108&.185&.224&.253&.27&.275&.295 \tabularnewline
&Neural net&.048&.038&.038&.034&.032&.031&.033 \tabularnewline
&Lasso with CV (TWI)&.044&.02&.014&.011&.007&.007&.046 \tabularnewline
&Ridge with CV (TWI)&.063&.031&.015&.012&.01&.008&0 \tabularnewline
&Lasso with CV (QSI)&.131&.17&.223&.248&.27&.265&.356 \tabularnewline
&Ridge with CV (QSI)&.214&.206&.144&.1&.048&.049&0 \tabularnewline
&Random forest (low regularization)&.107&.104&.117&.13&.172&.208&.007 \tabularnewline
&Random forest (high regularization)&.211&.167&.148&.134&.116&.089&.161 \tabularnewline
&Gradient boosting (low regularization)&.031&.032&.035&.04&.038&.039&.101 \tabularnewline
&Gradient boosting (high regularization)&.042&.046&.042&.038&.037&.03&0 \tabularnewline


==> Simul/sim_WZ/ssw_d_singlebest_folds2.tex <==
&OLS&.022&.094&.157&.208&.242&.248&.382 \tabularnewline
&Neural net&.001&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.031&.012&.009&.003&.002&.001&.002 \tabularnewline
&Ridge with CV (TWI)&.177&.039&.004&.002&.004&.006&0 \tabularnewline
&Lasso with CV (QSI)&.164&.234&.317&.338&.316&.256&.438 \tabularnewline
&Ridge with CV (QSI)&.257&.268&.13&.053&.009&.025&0 \tabularnewline
&Random forest (low regularization)&.119&.043&.021&.007&.002&0&0 \tabularnewline
&Random forest (high regularization)&.189&.226&.261&.275&.31&.35&.005 \tabularnewline
&Gradient boosting (low regularization)&.001&.003&.005&.012&.031&.059&.173 \tabularnewline
&Gradient boosting (high regularization)&.039&.081&.095&.103&.084&.054&0 \tabularnewline


==> Simul/sim_WZ/ssw_y_nnls1_folds2.tex <==
&OLS&.154&.159&.149&.124&.092&.059&0 \tabularnewline
&Neural net&.056&.046&.048&.049&.053&.066&.047 \tabularnewline
&Lasso with CV (TWI)&.041&.034&.03&.026&.027&.026&.092 \tabularnewline
&Ridge with CV (TWI)&.042&.047&.045&.039&.027&.018&.035 \tabularnewline
&Lasso with CV (QSI)&.234&.286&.306&.304&.291&.285&.554 \tabularnewline
&Ridge with CV (QSI)&.207&.212&.229&.275&.32&.347&.249 \tabularnewline
&Random forest (low regularization)&.12&.089&.092&.096&.117&.138&.019 \tabularnewline
&Random forest (high regularization)&.082&.068&.047&.037&.028&.024&.003 \tabularnewline
&Gradient boosting (low regularization)&.037&.039&.039&.036&.036&.03&0 \tabularnewline
&Gradient boosting (high regularization)&.026&.02&.015&.012&.008&.006&0 \tabularnewline


==> Simul/sim_WZ/ssw_y_singlebest_folds2.tex <==
&OLS&.07&.124&.101&.072&.034&.012&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.015&.014&.013&.009&.009&.011&0 \tabularnewline
&Ridge with CV (TWI)&.067&.058&.067&.063&.054&.039&0 \tabularnewline
&Lasso with CV (QSI)&.282&.383&.43&.424&.394&.38&.808 \tabularnewline
&Ridge with CV (QSI)&.261&.251&.281&.35&.441&.498&.192 \tabularnewline
&Random forest (low regularization)&.238&.111&.06&.042&.036&.033&0 \tabularnewline
&Random forest (high regularization)&.029&.019&.014&.009&.004&.003&0 \tabularnewline
&Gradient boosting (low regularization)&.013&.016&.019&.022&.023&.024&0 \tabularnewline
&Gradient boosting (high regularization)&.025&.024&.015&.009&.005&.001&0 \tabularnewline


==> Simul/sim_WZ/stw_d_nnls1_folds10.tex <==
&OLS&.119&.184&.227&.247&.244&.242&.168 \tabularnewline
&Neural net&.047&.044&.041&.039&.034&.033&.046 \tabularnewline
&Lasso with CV (TWI)&.048&.029&.024&.018&.015&.012&.097 \tabularnewline
&Ridge with CV (TWI)&.05&.021&.013&.014&.011&.008&.001 \tabularnewline
&Lasso with CV (QSI)&.152&.205&.241&.253&.263&.247&.402 \tabularnewline
&Ridge with CV (QSI)&.214&.16&.096&.064&.064&.067&.001 \tabularnewline
&Random forest (low regularization)&.1&.114&.129&.16&.21&.265&.009 \tabularnewline
&Random forest (high regularization)&.181&.144&.124&.114&.076&.054&.121 \tabularnewline
&Gradient boosting (low regularization)&.036&.04&.047&.044&.043&.042&.155 \tabularnewline
&Gradient boosting (high regularization)&.053&.059&.06&.047&.04&.03&.001 \tabularnewline


==> Simul/sim_WZ/stw_d_nnls1_folds2.tex <==
&OLS&.081&.129&.167&.199&.234&.251&.175 \tabularnewline
&Neural net&.056&.044&.046&.043&.041&.039&.05 \tabularnewline
&Lasso with CV (TWI)&.072&.044&.03&.029&.023&.017&.04 \tabularnewline
&Ridge with CV (TWI)&.073&.044&.023&.018&.014&.014&.005 \tabularnewline
&Lasso with CV (QSI)&.128&.155&.198&.218&.248&.247&.389 \tabularnewline
&Ridge with CV (QSI)&.176&.212&.177&.141&.079&.061&.019 \tabularnewline
&Random forest (low regularization)&.105&.097&.108&.112&.137&.165&.013 \tabularnewline
&Random forest (high regularization)&.22&.181&.151&.135&.126&.11&.147 \tabularnewline
&Gradient boosting (low regularization)&.035&.037&.041&.042&.045&.048&.157 \tabularnewline
&Gradient boosting (high regularization)&.053&.056&.058&.062&.054&.046&.005 \tabularnewline


==> Simul/sim_WZ/stw_d_singlebest_folds10.tex <==
&OLS&.03&.102&.161&.198&.193&.164&.087 \tabularnewline
&Neural net&.002&.001&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.046&.024&.016&.01&.004&.003&.006 \tabularnewline
&Ridge with CV (TWI)&.099&.015&.007&.011&.007&.002&0 \tabularnewline
&Lasso with CV (QSI)&.201&.286&.324&.312&.288&.214&.601 \tabularnewline
&Ridge with CV (QSI)&.259&.163&.051&.025&.042&.042&0 \tabularnewline
&Random forest (low regularization)&.092&.036&.015&.01&.004&.003&0 \tabularnewline
&Random forest (high regularization)&.187&.239&.261&.288&.313&.428&.001 \tabularnewline
&Gradient boosting (low regularization)&.005&.012&.026&.04&.079&.115&.305 \tabularnewline
&Gradient boosting (high regularization)&.078&.122&.138&.107&.07&.029&0 \tabularnewline


==> Simul/sim_WZ/stw_d_singlebest_folds2.tex <==
&OLS&.011&.042&.081&.112&.172&.205&.233 \tabularnewline
&Neural net&.007&.002&.001&.001&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.068&.042&.025&.025&.014&.006&0 \tabularnewline
&Ridge with CV (TWI)&.171&.082&.024&.013&.01&.012&0 \tabularnewline
&Lasso with CV (QSI)&.161&.203&.272&.307&.323&.29&.507 \tabularnewline
&Ridge with CV (QSI)&.181&.256&.202&.127&.036&.026&0 \tabularnewline
&Random forest (low regularization)&.156&.08&.05&.027&.011&.007&0 \tabularnewline
&Random forest (high regularization)&.18&.2&.219&.242&.277&.299&.049 \tabularnewline
&Gradient boosting (low regularization)&.005&.006&.011&.016&.029&.056&.211 \tabularnewline
&Gradient boosting (high regularization)&.06&.088&.116&.13&.128&.1&0 \tabularnewline


==> Simul/sim_WZ/stw_y_nnls1_folds10.tex <==
&OLS&.163&.159&.133&.1&.055&.029&0 \tabularnewline
&Neural net&.054&.052&.058&.052&.096&.069&.082 \tabularnewline
&Lasso with CV (TWI)&.044&.034&.034&.032&.028&.03&.059 \tabularnewline
&Ridge with CV (TWI)&.054&.049&.045&.032&.017&.011&.056 \tabularnewline
&Lasso with CV (QSI)&.239&.271&.266&.273&.269&.285&.597 \tabularnewline
&Ridge with CV (QSI)&.19&.235&.271&.316&.337&.358&.187 \tabularnewline
&Random forest (low regularization)&.099&.092&.104&.118&.14&.169&.018 \tabularnewline
&Random forest (high regularization)&.087&.048&.027&.021&.019&.02&0 \tabularnewline
&Gradient boosting (low regularization)&.039&.04&.047&.045&.035&.027&.001 \tabularnewline
&Gradient boosting (high regularization)&.03&.019&.016&.011&.005&.002&0 \tabularnewline


==> Simul/sim_WZ/stw_y_nnls1_folds2.tex <==
&OLS&.129&.161&.168&.154&.124&.094&0 \tabularnewline
&Neural net&.073&.052&.058&.05&.054&.07&.043 \tabularnewline
&Lasso with CV (TWI)&.051&.044&.037&.035&.033&.032&.122 \tabularnewline
&Ridge with CV (TWI)&.059&.052&.051&.048&.039&.029&.007 \tabularnewline
&Lasso with CV (QSI)&.205&.246&.27&.276&.272&.271&.474 \tabularnewline
&Ridge with CV (QSI)&.177&.193&.202&.241&.288&.312&.316 \tabularnewline
&Random forest (low regularization)&.146&.097&.095&.096&.108&.122&.031 \tabularnewline
&Random forest (high regularization)&.078&.083&.056&.04&.024&.02&.005 \tabularnewline
&Gradient boosting (low regularization)&.04&.04&.04&.041&.045&.041&.003 \tabularnewline
&Gradient boosting (high regularization)&.042&.031&.023&.019&.013&.009&0 \tabularnewline


==> Simul/sim_WZ/stw_y_singlebest_folds10.tex <==
&OLS&.108&.123&.087&.045&.012&.002&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.028&.018&.015&.014&.012&.017&0 \tabularnewline
&Ridge with CV (TWI)&.073&.072&.08&.065&.043&.022&0 \tabularnewline
&Lasso with CV (QSI)&.31&.374&.372&.382&.384&.396&.935 \tabularnewline
&Ridge with CV (QSI)&.232&.286&.338&.401&.47&.491&.065 \tabularnewline
&Random forest (low regularization)&.162&.071&.054&.048&.043&.038&0 \tabularnewline
&Random forest (high regularization)&.03&.011&.003&.001&.001&.001&0 \tabularnewline
&Gradient boosting (low regularization)&.02&.025&.037&.038&.035&.034&0 \tabularnewline
&Gradient boosting (high regularization)&.036&.02&.013&.006&.001&0&0 \tabularnewline


==> Simul/sim_WZ/stw_y_singlebest_folds2.tex <==
&OLS&.042&.109&.134&.111&.066&.035&0 \tabularnewline
&Neural net&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.034&.029&.021&.02&.015&.015&.003 \tabularnewline
&Ridge with CV (TWI)&.098&.072&.073&.071&.08&.063&0 \tabularnewline
&Lasso with CV (QSI)&.238&.319&.366&.378&.376&.383&.682 \tabularnewline
&Ridge with CV (QSI)&.217&.238&.246&.295&.364&.416&.314 \tabularnewline
&Random forest (low regularization)&.286&.147&.095&.07&.051&.044&0 \tabularnewline
&Random forest (high regularization)&.024&.027&.019&.008&.002&.002&0 \tabularnewline
&Gradient boosting (low regularization)&.019&.022&.021&.027&.035&.037&0 \tabularnewline
&Gradient boosting (high regularization)&.042&.036&.025&.02&.011&.004&0 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_candidate_f10.tex <==
&OLS (TWI)&-1810.9&267&605.1&2.9&-131.9&32.1 \tabularnewline
&OLS (QSI)&-3061.5&7054.9&-770&-7856.9&-1419.2&-6851.3 \tabularnewline
&Lasso with CV (TWI)&5943.6&3195.8&2589.1&1706.2&872.2&734.1 \tabularnewline
&Lasso with CV (QSI)&260.2&-322.1&-311.9&-551.8&-597.1&-239.8 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_candidate_f2.tex <==
&OLS (TWI)&-1133.5&-243.4&-198&-516.4&574.3&359.2 \tabularnewline
&OLS (QSI)&-2675.8&-3137.7&-3563.3&7023&-2604.8&-9974.5 \tabularnewline
&Lasso with CV (TWI)&7184.1&5485.8&3408.9&2998&2509.6&1848 \tabularnewline
&Lasso with CV (QSI)&911.3&191.9&-874.5&-628.5&-207.1&-286.3 \tabularnewline


==> Simul/sim_WZ_linear/bias_ddml_meta_f2.tex <==
&Short-stacking: CLS&2186.3&878.7&-463.4&-335.8&-96.4&-207.7 \tabularnewline
&Short-stacking: Single-best&2395.8&611.2&-628.4&-525.6&-187.5&-284.1 \tabularnewline
&Pooled stacking: CLS&1753.2&501.9&-706.5&-487.3&-173.1&-304.2 \tabularnewline
&Pooled stacking: Single-best&2161.3&729.3&-638&-480.8&-150.3&-230.2 \tabularnewline
&Stacking: CLS&1012.5&167.8&-713&-528&-198.9&-264.4 \tabularnewline
&Stacking: Single-best&2010.6&903.1&-573.3&-399.8&-97&-200.3 \tabularnewline


==> Simul/sim_WZ_linear/bias_olspds_f10.tex <==
&OLS QSI&-2113.4&-936.2&-806.4&-809.9&-677.2&-626.5 \tabularnewline
&OLS TWI&-1747.3&-479.9&13.2&-366&-320.3&-91.3 \tabularnewline
&Post double Lasso QSI c=0.5&381.6&-297.1&-204&-503.1&-571.6&-354.1 \tabularnewline
&Post double Lasso QSI c=1&-215.1&-1104.2&-639.4&-1063.2&-1000.5&-523.5 \tabularnewline
&Post double Lasso QSI c=1.5&8040.9&754.4&-1526.2&-2434.4&-2255.4&-1863.5 \tabularnewline
&Post double Lasso TWI c=0.5&3577.5&2490.3&2347.2&1748.3&1270.4&1197.5 \tabularnewline
&Post double Lasso TWI c=1&6270.2&3476.2&3453.1&2523.9&1702.4&1871.8 \tabularnewline
&Post double Lasso TWI c=1.5&14382.3&8943.3&6317.9&4802.2&3939&3094.5 \tabularnewline


==> Simul/sim_WZ_linear/bias_olspds_f2.tex <==
&OLS QSI&-2532.3&-1311.4&-1421.9&-961.6&-399&-282.2 \tabularnewline
&OLS TWI&-2100.3&-448&-936.5&-531.8&23.1&244.7 \tabularnewline
&Post double Lasso QSI c=0.5&-154.7&-120.1&-1019.8&-628.9&-50.5&-161.7 \tabularnewline
&Post double Lasso QSI c=1&-600.6&-1053&-1576.5&-1079&-485.1&-424.9 \tabularnewline
&Post double Lasso QSI c=1.5&7836.3&1064&-2253.4&-2434.8&-1644.7&-1698.3 \tabularnewline
&Post double Lasso TWI c=0.5&2869.2&2790.9&1635.4&1595.6&1767.6&1460.7 \tabularnewline
&Post double Lasso TWI c=1&5189.7&3966.8&2742&2328.1&2174.8&1975.8 \tabularnewline
&Post double Lasso TWI c=1.5&13651.1&9399.4&5610&4277&4150.8&3065.3 \tabularnewline


==> Simul/sim_WZ_linear/fullsample_ddml.tex <==
&OLS (TWI)&6796.682 \tabularnewline
&OLS (QSI)&4853.811 \tabularnewline
&Lasso with CV (TWI)&6780.161 \tabularnewline
&Lasso with CV (QSI)&5722.624 \tabularnewline


==> Simul/sim_WZ_linear/fullsample_meta.tex <==
&Pooled stacking: CLS&6009.779 \tabularnewline
&Pooled stacking: Single-best&5722.624 \tabularnewline
&Short-stacking: CLS&6044.902 \tabularnewline
&Short-stacking: Single-best&5722.396 \tabularnewline
&Stacking: CLS&6014.819 \tabularnewline
&Stacking: Single-best&5719.905 \tabularnewline


==> Simul/sim_WZ_linear/fullsample_olspds.tex <==
&OLS TWI&6751.907 \tabularnewline
&OLS QSI&5988.413 \tabularnewline
&Post double Lasso TWI c=0.5&6562.923 \tabularnewline
&Post double Lasso QSI c=0.5&5648.14 \tabularnewline
&Post double Lasso TWI c=1&6630.751 \tabularnewline
&Post double Lasso QSI c=1&4646.575 \tabularnewline
&Post double Lasso TWI c=1.5&7474.508 \tabularnewline
&Post double Lasso QSI c=1.5&4472.324 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_nnls1_folds10.tex <==
&OLS (TWI)&.002&.058&.055&.062&.069&.08&.111 \tabularnewline
&OLS (QSI)&0&0&0&0&.004&.007&.108 \tabularnewline
&Lasso with CV (TWI)&.264&.153&.125&.109&.11&.116&.234 \tabularnewline
&Lasso with CV (QSI)&.734&.789&.82&.829&.817&.796&.547 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_nnls1_folds2.tex <==
&OLS (TWI)&.016&.001&.061&.051&.05&.06&.091 \tabularnewline
&OLS (QSI)&.001&.038&0&0&0&0&.046 \tabularnewline
&Lasso with CV (TWI)&.376&.24&.165&.154&.124&.111&.167 \tabularnewline
&Lasso with CV (QSI)&.607&.722&.773&.795&.826&.829&.696 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.173&.064&.043&.04&.021&.017&0 \tabularnewline
&Lasso with CV (QSI)&.827&.936&.957&.96&.979&.983&1 \tabularnewline


==> Simul/sim_WZ_linear/psw_d_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.349&.169&.084&.069&.034&.022&0 \tabularnewline
&Lasso with CV (QSI)&.651&.831&.916&.931&.966&.978&1 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_nnls1_folds10.tex <==
&OLS (TWI)&.007&.054&.075&.074&.078&.081&.031 \tabularnewline
&OLS (QSI)&0&0&0&0&.005&.012&.093 \tabularnewline
&Lasso with CV (TWI)&.248&.208&.209&.193&.177&.164&.19 \tabularnewline
&Lasso with CV (QSI)&.744&.738&.716&.733&.74&.743&.686 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_nnls1_folds2.tex <==
&OLS (TWI)&.035&.001&.046&.053&.072&.079&.083 \tabularnewline
&OLS (QSI)&.005&.004&0&0&0&.001&.043 \tabularnewline
&Lasso with CV (TWI)&.272&.25&.221&.203&.19&.177&.12 \tabularnewline
&Lasso with CV (QSI)&.688&.746&.732&.743&.738&.744&.754 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.157&.092&.088&.074&.059&.053&0 \tabularnewline
&Lasso with CV (QSI)&.843&.908&.912&.926&.941&.947&1 \tabularnewline


==> Simul/sim_WZ_linear/psw_y_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.233&.165&.121&.094&.084&.075&.002 \tabularnewline
&Lasso with CV (QSI)&.767&.835&.879&.906&.916&.925&.998 \tabularnewline


==> Simul/sim_WZ_linear/ssw_d_nnls1_folds2.tex <==
&OLS (TWI)&.007&.007&.023&.035&.06&.079&.112 \tabularnewline
&OLS (QSI)&0&0&0&0&.001&.004&.069 \tabularnewline
&Lasso with CV (TWI)&.323&.203&.155&.136&.116&.104&.194 \tabularnewline
&Lasso with CV (QSI)&.67&.79&.822&.829&.823&.813&.625 \tabularnewline


==> Simul/sim_WZ_linear/ssw_d_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.289&.139&.084&.07&.039&.03&.006 \tabularnewline
&Lasso with CV (QSI)&.711&.861&.916&.93&.961&.97&.994 \tabularnewline


==> Simul/sim_WZ_linear/ssw_y_nnls1_folds2.tex <==
&OLS (TWI)&.011&.015&.032&.044&.065&.079&.085 \tabularnewline
&OLS (QSI)&.001&0&0&0&.003&.008&.061 \tabularnewline
&Lasso with CV (TWI)&.255&.228&.212&.188&.172&.159&.118 \tabularnewline
&Lasso with CV (QSI)&.732&.757&.756&.768&.759&.754&.736 \tabularnewline


==> Simul/sim_WZ_linear/ssw_y_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.215&.149&.127&.107&.095&.084&0 \tabularnewline
&Lasso with CV (QSI)&.785&.851&.873&.893&.905&.916&1 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_nnls1_folds10.tex <==
&OLS (TWI)&.005&.051&.049&.062&.081&.104&.121 \tabularnewline
&OLS (QSI)&0&0&0&.001&.005&.012&.107 \tabularnewline
&Lasso with CV (TWI)&.285&.178&.146&.128&.114&.111&.225 \tabularnewline
&Lasso with CV (QSI)&.709&.771&.804&.81&.799&.773&.548 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_nnls1_folds2.tex <==
&OLS (TWI)&.025&.001&.054&.047&.053&.064&.096 \tabularnewline
&OLS (QSI)&.003&.024&0&0&0&.001&.051 \tabularnewline
&Lasso with CV (TWI)&.381&.267&.19&.175&.144&.127&.16 \tabularnewline
&Lasso with CV (QSI)&.592&.708&.756&.778&.803&.807&.693 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.256&.135&.097&.075&.056&.05&.025 \tabularnewline
&Lasso with CV (QSI)&.744&.865&.903&.924&.944&.95&.975 \tabularnewline


==> Simul/sim_WZ_linear/stw_d_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.385&.24&.152&.132&.094&.072&.022 \tabularnewline
&Lasso with CV (QSI)&.615&.76&.848&.868&.906&.928&.978 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_nnls1_folds10.tex <==
&OLS (TWI)&.012&.055&.07&.079&.086&.098&.052 \tabularnewline
&OLS (QSI)&0&0&0&.002&.012&.021&.1 \tabularnewline
&Lasso with CV (TWI)&.255&.212&.208&.183&.164&.149&.165 \tabularnewline
&Lasso with CV (QSI)&.733&.734&.722&.737&.737&.732&.683 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_nnls1_folds2.tex <==
&OLS (TWI)&.044&.003&.048&.057&.074&.08&.085 \tabularnewline
&OLS (QSI)&.009&.003&0&0&0&.003&.055 \tabularnewline
&Lasso with CV (TWI)&.277&.259&.23&.211&.199&.182&.131 \tabularnewline
&Lasso with CV (QSI)&.67&.735&.722&.732&.726&.735&.729 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_singlebest_folds10.tex <==
&OLS (TWI)&0&0&0&0&.001&0&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.209&.146&.136&.113&.095&.084&0 \tabularnewline
&Lasso with CV (QSI)&.791&.854&.864&.886&.904&.916&1 \tabularnewline


==> Simul/sim_WZ_linear/stw_y_singlebest_folds2.tex <==
&OLS (TWI)&0&0&0&0&0&.001&0 \tabularnewline
&OLS (QSI)&0&0&0&0&0&0&0 \tabularnewline
&Lasso with CV (TWI)&.27&.207&.167&.142&.131&.113&.005 \tabularnewline
&Lasso with CV (QSI)&.73&.793&.833&.858&.868&.886&.995 \tabularnewline


==> partialinput.tex <==
\makeatletter
\newread\pin@file
\newcounter{pinlineno}
\newcommand\pin@accu{}
\newcommand\pin@ext{pintmp}
% inputs #3, selecting only lines #1 to #2 (inclusive)
\newcommand*\partialinput [3] {%
\IfFileExists{#3}{%
\openin\pin@file #3%
% skip lines 1 to #1 (exclusive)
\setcounter{pinlineno}{1}%
\@whilenum\value{pinlineno}<#1 \do{%
\read\pin@file to\pin@line%
\stepcounter{pinlineno}%
}%
% prepare reading lines #1 to #2 inclusive
\addtocounter{pinlineno}{-1}%
\let\pin@accu\empty%
\begingroup%
\endlinechar\newlinechar
\@whilenum\value{pinlineno}<#2 \do{%
% use safe catcodes provided by e-TeX's \readline
\readline\pin@file to\pin@line%
\edef\pin@accu{\pin@accu\pin@line}%
\stepcounter{pinlineno}%
}%
\closein\pin@file%
\expandafter\endgroup%
\scantokens\expandafter{\pin@accu}%
}{%
\errmessage{File `#3' doesn't exist!}%
}%
}
\makeatother

==> scopus_cites/mspe_levels.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Fri Jun 28 20:49:06 2024
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 58382.6 & 58226.2 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & OLS \& BERT &  & 58888.3 & 58294.9 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-lasso \& Unigrams &  & 58236.\phantom{0} & 58133.\phantom{0} &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-lasso \& BERT &  & 57268.4 & 57067.8 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-ridge \& Unigrams &  & 58265.8 & 58155.1 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & CV-ridge \& BERT &  & 57241.2 & 57078.5 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & XGBoost \& Unigrams &  & 68369.6 & 68987.3 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & XGBoost \& BERT &  & 67549.1 & 66907.5 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Random forest \& Unigrams &  & 59092.1 & 58955.7 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Random forest \& BERT &  & 60803.1 & 60570.6 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Neural net \& Unigrams &  & 63247.8 & 62674.\phantom{0} &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
   & Neural net \& BERT &  & 63371.9 & 63360.3 &  & 0.1 & 0.1 &  & 0.2 & 0.2 \\ 
  

==> scopus_cites/mspe_log.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Fri Jun 28 20:49:06 2024
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 1.341 & 1.336 &  & 0.058 & 0.058 &  & 0.166 & 0.166 \\ 
   & OLS \& BERT &  & 1.294 & 1.281 &  & 0.059 & 0.058 &  & 0.166 & 0.164 \\ 
   & CV-lasso \& Unigrams &  & 1.339 & 1.335 &  & 0.058 & 0.058 &  & 0.165 & 0.165 \\ 
   & CV-lasso \& BERT &  & 1.274 & 1.267 &  & 0.057 & 0.057 &  & 0.161 & 0.161 \\ 
   & CV-ridge \& Unigrams &  & 1.341 & 1.337 &  & 0.058 & 0.058 &  & 0.165 & 0.165 \\ 
   & CV-ridge \& BERT &  & 1.286 & 1.283 &  & 0.057 & 0.057 &  & 0.161 & 0.161 \\ 
   & XGBoost \& Unigrams &  & 1.439 & 1.415 &  & 0.075 & 0.073 &  & 0.196 & 0.192 \\ 
   & XGBoost \& BERT &  & 1.472 & 1.462 &  & 0.068 & 0.068 &  & 0.191 & 0.191 \\ 
   & Random forest \& Unigrams &  & 1.358 & 1.346 &  & 0.059 & 0.059 &  & 0.167 & 0.167 \\ 
   & Random forest \& BERT &  & 1.52\phantom{0} & 1.508 &  & 0.059 & 0.059 &  & 0.169 & 0.168 \\ 
   & Neural net \& Unigrams &  & 2.082 & 1.95\phantom{0} &  & 0.059 & 0.059 &  & 0.177 & 0.177 \\ 
   & Neural net \& BERT &  & 2.207 & 2.207 &  & 0.059 & 0.059 &  & 0.177 & 0.177 \\ 
  

==> scopus_cites/mspe_log_joined.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Fri Jun 28 20:49:06 2024
gap0 & learner & gap1 & y_X_Conventional & gap2 & D1_X_Conventional & gap3 & D2_X_Conventional \\ 
  & OLS \& Unigrams &  & \multicolumn{2}{c}{1.341} &  & \multicolumn{2}{c}{0.058} &  & \multicolumn{2}{c}{0.166} \\ 
   & OLS \& BERT &  & \multicolumn{2}{c}{1.294} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.166} \\ 
   & CV-lasso \& Unigrams &  & \multicolumn{2}{c}{1.339} &  & \multicolumn{2}{c}{0.058} &  & \multicolumn{2}{c}{0.165} \\ 
   & CV-lasso \& BERT &  & \multicolumn{2}{c}{1.274} &  & \multicolumn{2}{c}{0.057} &  & \multicolumn{2}{c}{0.161} \\ 
   & CV-ridge \& Unigrams &  & \multicolumn{2}{c}{1.341} &  & \multicolumn{2}{c}{0.058} &  & \multicolumn{2}{c}{0.165} \\ 
   & CV-ridge \& BERT &  & \multicolumn{2}{c}{1.286} &  & \multicolumn{2}{c}{0.057} &  & \multicolumn{2}{c}{0.161} \\ 
   & XGBoost \& Unigrams &  & \multicolumn{2}{c}{1.439} &  & \multicolumn{2}{c}{0.075} &  & \multicolumn{2}{c}{0.196} \\ 
   & XGBoost \& BERT &  & \multicolumn{2}{c}{1.472} &  & \multicolumn{2}{c}{0.068} &  & \multicolumn{2}{c}{0.191} \\ 
   & Random forest \& Unigrams &  & \multicolumn{2}{c}{1.358} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.167} \\ 
   & Random forest \& BERT &  & \multicolumn{2}{c}{1.52\phantom{0}} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.169} \\ 
   & Neural net \& Unigrams &  & \multicolumn{2}{c}{2.082} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.177} \\ 
   & Neural net \& BERT &  & \multicolumn{2}{c}{2.207} &  & \multicolumn{2}{c}{0.059} &  & \multicolumn{2}{c}{0.177} \\ 
  

==> scopus_cites/results_tab.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Fri Jun 28 20:49:06 2024
 OLS \& base controls & 0.022 & 0.226*** & -9.129** & 12.168*** \\ 
   & (0.03) & (0.017) & (4.438) & (3.045) \\ 
  PDS-lasso \& base controls & 0.025 & 0.231*** & -8.901** & 12.317*** \\ 
   & (0.03) & (0.017) & (4.431) & (3.045) \\ 
  PDS-lasso \& Unigrams & -0.056* & 0.106*** & -15.77*** & 2.844 \\ 
   & (0.029) & (0.017) & (4.283) & (3.053) \\ 
  PDS-lasso \& BERT & -0.074** & 0.092*** & -15.051*** & 2.125 \\ 
   & (0.029) & (0.017) & (4.428) & (3.053) \\ 
  OLS \& Unigrams & -0.052* & 0.103*** & -12.293** & 2.647 \\ 
   & (0.03) & (0.018) & (6.104) & (3.635) \\ 
  OLS \& BERT & -0.072** & 0.066*** & -8.686 & 1.454 \\ 
   & (0.029) & (0.017) & (6.242) & (3.655) \\ 
  CV-lasso \& Unigrams & -0.05* & 0.104*** & -12.388** & 2.648 \\ 
   & (0.03) & (0.018) & (6.116) & (3.621) \\ 
  CV-lasso \& BERT & -0.069** & 0.069*** & -9.928 & 2.209 \\ 
   & (0.029) & (0.017) & (6.142) & (3.648) \\ 
  CV-ridge \& Unigrams & -0.051* & 0.102*** & -12.383** & 2.077 \\ 
   & (0.03) & (0.018) & (6.115) & (3.627) \\ 
  CV-ridge \& BERT & -0.067** & 0.075*** & -9.86 & 2.056 \\ 
   & (0.029) & (0.017) & (6.155) & (3.636) \\ 
  XGBoost \& Unigrams & -0.065** & 0.073*** & 37.984*** & 23.481*** \\ 
   & (0.03) & (0.02) & (6.655) & (3.629) \\ 
  XGBoost \& BERT & -0.07** & 0.073*** & 9.473 & 8.922** \\ 
   & (0.031) & (0.021) & (7.306) & (3.796) \\ 
  Random forest \& Unigrams & -0.103*** & 0.044** & 0.444 & 5.255 \\ 
   & (0.029) & (0.017) & (6.098) & (3.623) \\ 
  Random forest \& BERT & -0.106*** & 0.055*** & 8.919 & 10.869*** \\ 
   & (0.031) & (0.018) & (6.148) & (3.667) \\ 
  Neural net \& Unigrams & -0.05 & 0.005 & -16.867*** & -9.791*** \\ 
   & (0.036) & (0.021) & (6.317) & (3.647) \\ 
  Neural net \& BERT & -0.047 & -0.014 & -16.979*** & -10.31*** \\ 
   & (0.038) & (0.022) & (6.316) & (3.643) \\ 
  Single-best \& stacking & -0.07** & 0.072*** & -10.204* & 2.274 \\ 
   & (0.029) & (0.017) & (6.123) & (3.65) \\ 
  CLS \& stacking & -0.071** & 0.063*** & -9.485 & 1.971 \\ 
   & (0.029) & (0.017) & (6.103) & (3.635) \\ 
  Single-best \& short-stacking & -0.069** & 0.07*** & -9.916 & 2.254 \\ 
   & (0.029) & (0.017) & (6.143) & (3.643) \\ 
  CLS \& short-stacking & -0.07** & 0.062*** & -9.529 & 1.615 \\ 
   & (0.029) & (0.017) & (6.099) & (3.628) \\ 
  

==> scopus_cites/weights_levels.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Fri Jun 28 20:49:06 2024
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 0.206 & 0.193 &  & 0.105 & 0.135 &  & 0.122 & 0.121 \\ 
   & OLS \& BERT &  & 0.205 & 0.209 &  & 0.102 & 0.099 &  & 0.165 & 0.179 \\ 
   & CV-lasso \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.062 & 0.002 &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-lasso \& BERT &  & 0.304 & 0.344 &  & 0.34\phantom{0} & 0.519 &  & 0.194 & 0.246 \\ 
   & CV-ridge \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-ridge \& BERT &  & 0.032 & 0.\phantom{000} &  & 0.359 & 0.19\phantom{0} &  & 0.338 & 0.264 \\ 
   & XGBoost \& Unigrams &  & 0.06\phantom{0} & 0.065 &  & 0.018 & 0.018 &  & 0.019 & 0.016 \\ 
   & XGBoost \& BERT &  & 0.092 & 0.099 &  & 0.014 & 0.015 &  & 0.028 & 0.038 \\ 
   & Random forest \& Unigrams &  & 0.134 & 0.124 &  & 0.021 & 0.047 &  & 0.155 & 0.156 \\ 
   & Random forest \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & Neural net \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & Neural net \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
  

==> scopus_cites/weights_log.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Fri Jun 28 20:49:06 2024
gap0 & learner & gap1 & y_X_Conventional & y_X_Short & gap2 & D1_X_Conventional & D1_X_Short & gap3 & D2_X_Conventional & D2_X_Short \\ 
  & OLS \& Unigrams &  & 0.1\phantom{00} & 0.069 &  & 0.113 & 0.155 &  & 0.135 & 0.114 \\ 
   & OLS \& BERT &  & 0.35\phantom{0} & 0.368 &  & 0.09\phantom{0} & 0.106 &  & 0.174 & 0.196 \\ 
   & CV-lasso \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.049 & 0.013 &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-lasso \& BERT &  & 0.119 & 0.102 &  & 0.363 & 0.396 &  & 0.129 & 0.166 \\ 
   & CV-ridge \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & CV-ridge \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.361 & 0.31\phantom{0} &  & 0.383 & 0.329 \\ 
   & XGBoost \& Unigrams &  & 0.217 & 0.236 &  & 0.008 & 0.008 &  & 0.017 & 0.028 \\ 
   & XGBoost \& BERT &  & 0.171 & 0.174 &  & 0.016 & 0.01\phantom{0} &  & 0.033 & 0.035 \\ 
   & Random forest \& Unigrams &  & 0.047 & 0.055 &  & 0.02\phantom{0} & 0.026 &  & 0.149 & 0.151 \\ 
   & Random forest \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.001 & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & Neural net \& Unigrams &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
   & Neural net \& BERT &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} &  & 0.\phantom{000} & 0.\phantom{000} \\ 
  
